Efficient Algorithms for Extreme Bandits

In this paper, we contribute to the Extreme Bandit problem, a variant of Multi-Armed Bandits in which the learner seeks to collect the largest possible reward. We first study the concentration of the maximum of i.i.d random variables under mild assumptions on the tail of the rewards distributions. This analysis motivates the introduction of Quantile of Maxima (QoMax). The properties of QoMax are sufficient to build an Explore-Then-Commit (ETC) strategy, QoMax-ETC, achieving strong asymptotic guarantees despite its simplicity. We then propose and analyze a more adaptive, anytime algorithm, QoMax-SDA, which combines QoMax with a subsampling method recently introduced by Baudry et al. (2021). Both algorithms are more efficient than existing approaches in two aspects (1) they lead to better empirical performance (2) they enjoy a significant reduction of the memory and time complexities.

==> MoMax_ETC.tex <==
\newpage

\section{MoMAX-ETC}

\subsection{MoMax}

\subsubsection{Properties of the maximum of $n$ random variables}

Consider a collection of i.i.d random variables $(X_1, \dots, X_n)$ 
with cdf $F_X$ and denote $G_X=1-F_X$ and 
$X_n^+ = \max \{X_1, \dots, X_n \}$. Then the cdf of $X_n^+$ 
is immediately derived from F, for any $x \in \R$,

\begin{equation}\label{eq::prob_inf}\bP(X_n^+ \leq x)= F_X(x)^n \leq \exp(-n G_X(x)) \;.
\end{equation}

We see that $\bP(X_n^+ \geq x)$ have a more complicated form. 
However, when $x$ is large a simple union bound is actually quite tight,
\begin{equation}
\label{eq::prob_sup}
\bP(X_n^+ \geq x)\leq \sum_{i=1}^n 
\bP(X_i\geq x) = n G(x) \;.
\end{equation}
Using Equation~\ref{eq::prob_inf} and \ref{eq::prob_sup}, for two samples $(X_1, \dots, X_n)$ and $(Y_1, \dots, Y_n)$ with respective maxima $X_n^+$ and $Y_n^+$ we want to upper bound the probability $\bP(X_n^+ \leq Y_n^+)$ by finding a suitable sequence $x_n$ aimed at minimizing $\max(\bP(X_n^+ \leq x_n), \bP(Y_n^+ \geq x_n))$. We start by providing a result for some parametric assumptions on the tail of the distributions, showing that in this case an upper bound in $\cO((\log n)^{l+1} n^{-l})$ can be obtained for some $l>0$.

\begin{definition}
Arm $k$ is exponential if $G_k(x) \sim a_k e^{-\lambda_k x}$
\end{definition}

{\color{blue} better statement of this result for making it clear that $X$ is the distribution with the heavier tail}

\begin{lemma}[Concentration for exponential and polynomial tails]
\label{lem::concent_expoly_app} 
Consider two tails that are either polynomial or exponential 
with parameters $\lambda_1 < \lambda_2$. Let $X_n^+$ 
and $Y_n^+$ denote respectively the maximum of $n$ i.i.d 
random variables drawn respectively from $\nu_X$ 
(with parameeter $\lambda_1$) and $\nu_Y$ 
(with parameter ($\lambda_2$). Then, 
there exists some sequence $x_n$ for which 
	\[
	\max\left\{\bP\left(X_n^+ \leq x_n\right), 
	\bP\left(Y_n^+\geq x_n \right) \right\} 
	= \cO\left(\frac{(\log n)^{\lambda_2/\lambda_1}}{
	n^{\frac{\lambda_2}{\lambda_1}-1}}\right) \;.
	\]
\end{lemma}

\begin{proof}
The key of the proof is to consider $x_n$ "slightly" 
below $G_X^{-1}(1/n)$. Consider the exponential tails first: we say 
that the tails are exponential if there exist parameters 
$(a_1, a_2, \lambda_1, \lambda_2)$ such 
as for $x$ large enough, $G_X(x)=a_1 \exp(-\lambda_1 x)$ 
and $G_Y(x)=a_2 \exp(-\lambda_2 x)$, 
with $\lambda_1 < \lambda_2$. The closest 
equivalent of the gap in classical bandits is 
the quantity $l_{12}= \frac{\lambda_2}{\lambda_1}-1$. Then, we 
choose 
\[
x_n = \frac{1}{\lambda_1}\left(\log n + \log(a_1) 
- \log(l_{12} \log n)\right) \;.
\]
	
	We now simply compute $G_X(x_n)$ and $G_Y(x_n)$. First,	
	\begin{align*}
	G_X(x_n) &= a_1 \exp(-(\log n + \log a_1 - \log(l_{12})\log n))\\
	& = \frac{l_{12}(\log n)}{n} \;.
	\end{align*}
	Then, 
	\begin{align*}
	G_Y(x_n) &= 
	a_2 \exp\left(-\frac{\lambda_2}{\lambda_1}
	\left(\log n + \log a_1 - \log(l_{12}\log n\right)\right) 
	\\
	& = \frac{1}{n^{\frac{\lambda_2}{\lambda_1}}} 
	\times (l_{12} \log n)^{\frac{\lambda_2}{\lambda_1}}
	\times\frac{a_2}{a_1^\frac{\lambda_2}{\lambda_1}}
	\end{align*}

	So finally, using Equation~\ref{eq::prob_inf} and \ref{eq::prob_sup} we obtain 
	\[
	\bP\left(Y_n^+ \geq x_n\right) 
	= \cO\left(\frac{(\log n )^{\frac{\lambda_2}{\lambda_1}}}
	{n^{l_{12}}}\right) \quad \text{and} \quad 
	\bP\left(X_n^+ \leq x_n\right) \leq \frac{1}{n^{l_{12}}} \;, 
	\]
which gives the result.
	

Now we consider polynomial tails, that we parametrize this time as $G_X(x)=a_1 x^{-\lambda_1}$ and $G_Y(x)=a_2 x^{-\lambda_2}$. We follow the exact same proof, this time with the sequence 
\[
x_n = (a_1 n )^\frac{1}{\lambda_1} 
\times (l_{12} \log n)^{-\frac{1}{\lambda_1}} \;,
\]
with the same definition of $l_{12}$. We again have $\exp(-nG_X(x_n))=n^{-l_{12}}$, and $nG_2(x_n) = \cO\left(\frac{(\log n )^{\frac{\lambda_2}{\lambda_1}}}{n^{l_{12}}}\right)$, giving the result.

\end{proof}

\begin{remark}
	An open question could be to determine if there exists a better rate, possibly by directly computing $\bP(X_n^+ \leq Y_n^+)$ instead of using this decomposition. Indeed, with this technique it appears clearly that the order cannot be improved as the upper bounds would evolve in an opposite direction when changing $x_n$. Could be interesting to verify this with plots.
\end{remark}

Lemma~\ref{lem::concent_expoly} will be crucial to design and evaluate the performance of the MoMax-ETC strategy. It is sufficient to handle all the cases for which algorithms exist in the literature. More precisely, existing solutions work only when the growth rates of the maxima can be clearly distinguished, e.g when tails are exponential or Pareto with different rates $\lambda_X \neq \lambda_Y$. In the following, we try to relax this condition and study a looser property for tail comparison.

%{\cxolor{blue} est-ce qu'on aurait pas envie de dire asymptoticallt dominating arm-tail pour qu'on comprenne un peu mieux que c'est au niveau des queues qu'on s'intéresse aux distributions.}
\begin{definition}[Asymptotically dominating arm]
Let $F_X$ and $F_Y$ be the cumulative distribution 
functions of two distributions $\nu_X$ and $\nu_Y$. 
	We say that $\nu_X$ dominates $\nu_Y$ asymptotically 
	if there exists some constant $C>1$ and some 
	$x \in \R$ satisfying $\forall y \geq x$, $G_X(y) > C G_Y(y)$. 
	We then denote $\nu_X \succ \nu_Y$.
\end{definition}

\begin{lemma}[Concentration under Asymptotic dominance]\label{lem::prob_dominance_app}
	Consider two distributions $\nu_X$ and $\nu_Y$ satisfying $\nu_X \succ \nu_Y$. Let $X_n^+$ and $Y_n^+$ denote respectively the maximum of $n$ i.i.d random variables drawn respectively from $\nu_X$ and $\nu_Y$. Then, there exists some $\epsilon>0$ and some sequence $u_n$ satisfying $\bP(X_n^+\leq u_n) \leq 1/2-\epsilon$ and $\bP(Y_n^+\geq u_n) \leq 1/2-\epsilon$ for $n$ large enough.
\end{lemma}

\begin{proof}
We start by considering $v_n = F_X^{-1}((1/2)^{1/n})$. By construction, this sequence then satisfies $\bP(X_n^+\leq v_n)=1/2$, and for $n$ large enough the condition holds in $v_n$. We now consider

\begin{align*}
\bP(Y_n^+ \leq v_n) & = F_Y(v_n)^n \\
& =(1-G_Y(v_n))^n \\
& \color{blue}{\geq (1- \frac{1}{C} G_X(v_n))^n} \\
& = \left(1-\frac{1}{C} \left(1-\left(\frac{1}{2}\right)^{1/n}\right)\right)^n \;. 
\\
\end{align*}
{\color{blue}question par rapport à la ligne en bleue: ici tu as utilisé que $v_n$ tend vers +  infiny donc existee n large enough pour etre dans lee régime de domination asymptotique c'est ça ?}


Now we can consider the asymptotic behavior of this quantity, using first that $1- \frac{1}{2^{1/n}} \sim \frac{\log 2}{n}$, and deducing then that \[\left(1-
\frac{1}{C} \left(1-\left(\frac{1}{2}\right)^{1/n}\right)\right)^n \sim \frac{1}{2^{\frac{1}{C}}}>\frac{1}{2} \;.\]

So for $n$ large enough we have both $\bP(X_n^+ \leq v_n)=1/2$ and $\bP(Y_n^+\leq v_n)\geq 1/2+\epsilon'$ for some $\epsilon'$ that depends on $C$. As there is a strictly positive gap between these two quantities, we can find some $\epsilon>0$ and a sequence $u_n$ satisfying both $\bP(X_n^+ \leq u_n)=1/2-\epsilon$ and $\bP(Y_n^+\leq u_n) \geq 1/2 + \epsilon$. The maximum possible value for $\epsilon$ depends only of the parameter $C$. This concludes the proof.
\end{proof} 

\begin{remark} We could ask ourselves if it is possible to obtain the same result with an even stronger condition, for instance only assuming $G_1(x)>G_2(x)$ for $x$ large enough. However, with this assumption it is possible to build pathological cases, such as defining $G_1(x)=G_2(x)\left(1+\frac{1}{x}\right)$. With the same analysis as the proof of Lemma~\ref{lem::prob_dominance}, by replacing $C= 1+\frac{1}{v_n}$ we would obtain $2^{-\frac{v_n}{v_n+1}} \rightarrow_{n \rightarrow + \infty} 1/2$. Logically, the two tails because impossible to distinguish when $n\rightarrow + \infty$. 
\end{remark}

\subsubsection{Concentration of the MoMax} 

\begin{lemma}[Concentration of MoMax]
\label{lem::MoMax_concentration_appendix}
Consider a sample of $m \in \N$ batches containing 
$n\in \N$ observations each. The $n\times m$ 
observations $(X_1^1, \dots, X_n^m)$ are i.i.d and 
drawn from a distribution $\nu_X$. For all $i \in [1, m]$ 
we denote $X_{n}^{i, +}$ as the maximum 
over the $n$ observations of the $i$-th batch, 
and $\bar X_n^+$ as the median of $(X_{n}^{i, +})_{i \leq m}$, that 
we call "Median of Maxima" (MoMax) of the 
sample. Then, for any $(x, y) \in \R^2$ satisfying 
respectively $\bP(X_n^{1, +} \geq x) < 1/2$ 
and $\bP(X_n^{1, +} \leq y) < 1/2$, it holds that 
	\[
	\bP(\bar X_n^+ \geq x) \leq 
	\exp(-m \times\kl(1/2, \bP(X_n^{1, +}\geq x))) \;,
	\]
	and  
	\[
	\bP(\bar X_n^+ \leq y) \leq 
	\exp(-m \times \kl(1/2, \bP(X_n^{1, +}\leq y))) \;,
	\]
where for $(p, q) \in (0, 1]$, $\kl(p, q)= p\log(p/q)+(1-p) \log((1-p)/(1-q))$, is the KL-divergence between two Bernoulli distributions with parameters $p$ and $q$.
\end{lemma}

\begin{proof}
Using the same kind of demonstration as \cite{bubeck_heavy} for the \textit{Median of Means} estimator, we use the concentration of Bernoulli random variables. The intuition is the following: if the median of the samples is larger (resp. smaller) than some $x \in \R$, then it holds that at least half of the batch estimators are larger than $x$ (resp. smaller), which gives $\sum_{i=1}^m \ind(X_n^{i, +} \geq x) \geq \lceil m/2 \rceil$. Hence, we can use the classical Chernoff concentration for Bernoulli random variables

\begin{align*}
\bP(\bar X_n^+ \geq x) &\leq \bP\left(\sum_{i=1}^{m} \ind\left(X_{n}^{i, +} \geq x \right) \geq \left\lceil \frac{m}{2}\right\rceil\right) \\
& \leq \exp\left(-m \times \kl\left(1/2, \bP(X_n^{1,+} \geq x)\right)\right) \;, 
\end{align*}

which holds if $\bP(X_n^+ \geq x) < 1/2$. The second result is directly proved using the exact same argument, since $\bP(X_n^+ \leq y) < 1/2$.
\end{proof}


\begin{corollary}\label{corr::prob_momax_lose}

Consider $\bar X_n^+$ and $\bar Y_n^+$ the MoMax of two samples of sizes $m \times n$ drawn respectively from distributions $\nu_X$ and $\nu_Y$. Then,

\begin{enumerate}
	\item If $\nu_X$ and $\nu_Y$ satisfy the condition of 
	Lemma~\ref{lem::concent_expoly}, then \textbf{for any} 
	$\epsilon>0$ there exists $n_0$ %large enough satisfying for any 
	such that for any
	$n\geq n_0$, 
	\[
	\bP\left(\bar X_n^+ \leq \bar Y_n^+\right) 
	\leq 2 \exp(-m\times \kl(1/2, \epsilon)) \;.
	\] 
	\item If $\nu_X$ and $\nu_Y$ satisfy the 
	condition of Lemma~\ref{lem::prob_dominance}, then 
	\textbf{there exists} some $\epsilon>0$ and $n_0$ %large enough
	such that 
	for any $n \geq n_0$, 
	\[
	\bP\left(\bar X_n^ + \leq \bar Y_n^+\right) 
	\leq 2 \exp(-m\times \kl(1/2, 1/2-\epsilon))\;.
	\]
\end{enumerate}
\end{corollary}

\begin{proof}
Denote $X_n^+$ and $Y_n^+$ the respective maxima of a single batch of size $n$ drawn from $\nu_X$ and $\nu_Y$. 

Under the assumptions of Lemma~\ref{lem::concent_expoly}, there exists a sequence $x_n$ satisfying 
{\color{blue}typo ligne d'en dessous j'imagine que ça doit être un max et qu'il n'y a pas le terme en $\bP(X_n)$}
$\bP(X_n)\left\{\bP\left(X_n^+ \geq x_n\right), \bP\left(Y_n^+\leq x_n \right) \right\} = \cO\left(\frac{(\log n)^{\lambda_2/\lambda_1}}{n^{\frac{\lambda_2}{\lambda_1}-1}}\right) \rightarrow_{n \rightarrow + \infty} 0$. Hence, for any $\epsilon >0$ for $n$ large enough the probabilities are both smaller than $\epsilon$. We then simply notice that $\bP(\bar X_n^+ \leq \bar Y_n^+) \leq \bP(\bar X_n^+ \leq x_n) + \bP(\bar Y_n^+ \geq x_n)$, which gives the result by direct application of Lemma~\ref{lem::MoMax_concentration}.

Similarly, Lemma~\ref{lem::prob_dominance} ensures the existence of some sequence $x_n$ and some $\epsilon>0$ satisfying $\max\left\{\bP\left(X_n^+ \geq x_n\right), \bP\left(Y_n^+\leq x_n \right)\right\} \leq 1/2-\epsilon$, for $n$ large enough. 
Following the reasoning from the previous case, we obtain the result.
%The result is then direct, with the same reasoning as for the first statement.
\end{proof}

\begin{remark}

$\kl(1/2, \epsilon_n) \approx 1/2 \log(1/\epsilon_n) - \log 2$, so if we have $\epsilon_n \sim n^{-\ell}$ like the concentration for the semi-parametric tails we actually have an upper bound in $\exp(-m (\ell \log(n)-\log 2))$. This is actually more logical than in the other size: with a strong concentration or a large sample size we can reduce the batch size required!
\end{remark}	

\subsection{Upper bound on the extremal regret}

\begin{theorem}[Regret of ETC in Extreme Bandits]
\label{th::regret_ETC}
	Let $\pi$ be an Explore-Then-Commit policy requiring 
	$N_0(T)$ samples for each arm before 
	committing to a single arm. Consider any bandit 
	problem $\nu=(\nu_1, \dots, \nu_K)$ with an asymptotically 
	dominating arm $\nu_1$, and denote $(X_1, \dots, X_n, \dots)$ 
	the observations sequentially collected from 
	this arm during the game. When $T$ is large enough 
	the extreme regret of ETC satisfies
	\begin{align*}
	\cR_{T}^\pi &= \bE\left[\max_{n \leq T} X_n\right] - 
	\bE\left[\max_{t \leq T} X_{N_{I_t}(t)}^{I_t}\right] 
	\\
	& \leq \bE\left[\max_{n \leq T} X_n\right]  
	- \bE\left[\max_{n \leq T-KN_0(T)} X_n\right] 
	+\bP(I_T\neq 1)\bE\left[\max_{n \leq T-KN_0(T)} X_n\right] 
	\\
	& \leq \underbrace{\bE\left[\max_{n \leq T} X_n\right]  - 
	\bE\left[\max_{n \leq T-KN_0(T)} X_n
	\right]}_{\text{Exploration Cost}} 
	+ 
	\underbrace{\bP(I_T\neq 1)\bE\left[\max_{n 
	\leq T} X_n\right]}_{\text{wrong 
	arm picked error}} \;.
	\end{align*}
\end{theorem}

\begin{proof}
	The ETC simplifies a lot the study of the extremal regret, as we can separate the explore and commit phase in the analysis. First, an exact decomposition of the expected value of the policy is 
	\[
	\bE\left[\max_{t \leq T} X_{N_{I_t}(t)}^{I_t}\right] 
	= \bE\left[\max \left\{ \max_k \max_{n \leq N_0(T)} X_n^k 
	, \max_{n=[N_0(T),T-(K-1)N_0(T)]} X_n^{I_T}\right\}\right] \;.
	\]
	
	We obtain a trivial lower bound by simply ignoring the exploration phase, and further proceed by only considering the event when the arm picked for the exploitation phase is the best arm
	
	\begin{align*}
	\bE\left[\max_{t \leq T} X_{N_{i_t}(t)}^{I_t}\right] &\geq \bE\left[\max_{n=[N_0(T),T-(K-1)N_0(T)]} X_n^{I_T} \ind(I_T=1)\right] \\
	&= \bE\left[\max_{n=[N_0(T),T-(K-1)N_0(T)]} X_n \ind(I_T=1)\right] \\
	& = \bP(I_T=1) \bE\left[\max_{n=[N_0(T),T-(K-1)N_0(T)]} X_n\right] \\
	& =\bP(I_T=1) \bE\left[\max_{n=[1,T-KN_0(T)]} X_n\right] \; \\
	&=  \bE\left[\max_{n \leq T-KN_0(T)} X_n
	\right] - \bP(I_T\neq 1)  
	\bE\left[\max_{n \leq T-KN_0(T)} X_n
	\right]  \\
	& \geq \bE\left[\max_{n \leq T-KN_0(T)} X_n
	\right] - \bP(I_T\neq 1)  
	\bE\left[\max_{n \leq T} X_n
	\right] \;.
	\end{align*}
	
	{\color{blue} pour la première ligne utilisation du fait que les distributions sont à valeurs positives pour faire apparaître l'indicatrice ?
	Autre remarque, est-ce que les indices devraient aller jusuq'à $T- (K-1)
	N_0(T) -1$ plutôt ? (j'avoue que je pinaille)}
	
There second equality holds because the fact that arm $1$ is chosen by the algorithm after the exploration phase is independent of the rewards that are available for arm $1$ in the exploitation phase. This concludes the proof.
\end{proof}



\paragraph{Examples: Polynomial and Logarithmic tails} 
From \cite{bhatt2021extreme} Equation (10), for a polynomial tail with 
rate $\alpha$ we obtain 
\[
\frac{\bE[\max_{n \leq T-KN_0(T)} X_n]}{\bE[\max_{n \leq T} X_n]} 
\sim \left(1-\frac{KN_0(T)}{T}\right)^\frac{1}{\alpha} \;, 
\]
or 

\[
\bE \left[\max_{n \leq T-KN_0(T)} X_n\right]-\bE[\max_{n \leq T} X_n] 
= (cT)^{1/\alpha}\times \left[1-\left(1-\frac{KN_0(T)}{T}\right)^{1/\alpha}\right]\sim \frac{C^{1/\alpha} K N_0(T)}{\alpha T^{1-1/\alpha}} 
\]

For a logarithmic tail $a e^{-\lambda x} $, 
we have 
{\color{red} ça vient d'où ça ?}
\[
\frac{\bE[\max_{n \leq T-KN_0(T)} X_n]}{\bE
[\max_{n \leq T} X_n]} \sim 
\frac{\log(T-KN_0(T))+\log a}{\log T + \log a} = 1 
+ \frac{\log\left(1-K\frac{N_0(T)}{T}\right)}{\log T 
+ \log a} \;, 
\]
or 
\[
\bE\left[\max_{n \leq T-KN_0(T)} X_n\right]
-\bE[\max_{n \leq T} X_n] = 
-\frac{\log\left(1-\frac{KN_0(T)}{T}\right)}{\lambda} 
\sim \frac{K N_0(T)}{\lambda T} \;.
\]

Hence, we see that the exploration cost vanishes in both cases if $N_0(T) = o(T^\delta)$ for any $\delta>0$. The exponential tails are less restrictive as $N_0(T)=o(T)$ is enough.

{\color{red} est-ce qu'on veut rajouter le statement de l'espeerance du max avec des distrib exponentielles pour justifier le statement de la ligne au dessus}

%{\color{blue} TODO Yo: j'ai pas encore checké cette partie là (au dessus).}

We now consider specifically the probability 
$\bP(I_T\neq 1)$ of MoMax-ETC. For 
simplicity we denote by $\bar X^{k, +}$
the MoMax estimator of arm  $k$ at the end of 
the exploration phase. Here, we assume either the 
tail assumptions of Lemma~\ref{lem::concent_expoly} 
or Lemma~\ref{lem::prob_dominance} and denote simply 
as $(m_T, n_T)$ the batch size and sample size used 
in MoMax. We have
\begin{align*}
\bP(I_T \neq 1) =& \sum_{k=2}^K \bP(I_T=k) \\
\leq & \sum_{k=2}^K \bP(\bar X^{1, +} \leq \bar X^{k, +}) \;.
\end{align*}

We then deduce from Corollary~\ref{corr::prob_momax_lose} 
that under assumptions of Lemma~\ref{lem::concent_expoly}, for 
any $\epsilon>0$ if $n_T$ is large enough we obtain 
\[
\bP(I_T \neq 1) \leq 2K \exp(-m_T\kl(1/2, \epsilon)) \;.
\]

Similarly, under the assumptions of 
Lemma~\ref{lem::prob_dominance} there exists 
some $\epsilon>0$ such that if $n_T$ is large enough we obtain 
\[
\bP(I_T \neq 1) \leq 2K \exp\left(-m_T\kl(1/2, 1/2-\epsilon)\right) \;.
\]

{\color{blue} pourquoi c'est $n_T$ que tu tunes ici ? c'est $m_T$ le nombre de batch sur lequel on a envie de jouer ici non?}

In the first case it suffices to choose $n_T = \frac{\log T}{\kl(1/2, \epsilon)}$ to obtain a probability of order $T^{-1}$, and $\epsilon$ can be chosen by the learner. In the second case $\epsilon$ is not known by the learner and so we have to choose $m_T$ satisfying $\log T = o(m_T)$ to obtain an upper bound of $T^{-1}$ asymptotically.


\begin{remark}[Regret of ExtremeHunter]
The regret of ExtremeHunter is of order $\bE[R_T] = \bE[\max_T X_n] \times \cO\left(T^{-\frac{b}{(b+1)\alpha^\star}}\right)$. This quantity is not vanishing when $T\rightarrow +\infty$ because it provides a scaling in $T^\frac{1}{(b+1)\alpha^*}$. On the other hand, the interest of the analysis of ExtremeHunter is that it provide an upper bound on the expected number of pulls of sub-optimal arms, of order $\cO\left(\right)$. 

Note that there is an inconsistency between different notations in the paper and in the code. Is $\log^2(n) = \log \log n $ ? It seems that Mastane thinks so. If so why do they write $\exp(-\log^2(n))$ in $\delta$ and not $1/\log(n)$? The value of $N$ is like $\cO(\log n)^{4+2/b}$, because of two conditions: one with a $\log^2(n)$ and the other with a $\log(n)^2$. If we take $\log^2(n)$ as $(\log(n))^2$ we indeed need $4+2/b$, if it is $\log\log$ then we need $(\log \log n)^4$ and $\log(n)^{2+1/b}$... which is the value of $N$ Michal put in the code... 
{\color{green}also check guaranties données dans le papier de Mastane pour le regret de ExtremeHunter histoire de voir si ils ont un résultat plus fort, il me semble que oui}

\end{remark}

==> QoMax_ETC.tex <==
\section{MoMAX-ETC}

We first propose MoMax-ETC, a simple and efficient algorithm for Extreme Bandits, with strong theoretical guarantees. The idea is simple:
\begin{enumerate}
	\item Samples each arm $N_0(T) = n_T \times m_T$ times, and store the data in $m_T$ batches of $n_T$ samples. We can suggest for instance $N_0(T)= \Omega((\log T)^2)$.
	\item Compute the MoMax estimator of each arm: Consider the $\frac{1+\epsilon}{\log 2} \log T$ batches of $\frac{1+\epsilon}{\log 2} \log T$ samples (could be less actually, any size that $\rightarrow + \infty$).
	\item Commit to the arm with best MoMax until time $T$.
\end{enumerate}

There are several advantages:
\begin{itemize}
	\item Sample size is deterministic: does not require tuning, only the parameter $\epsilon$ that could technically be as small as we want (see analysis).
	\item Non-Parametric assumptions on the tails of the distributions.
	\item Computation of the index is efficient: for single batches, online tracking of the maximum (cost one numeric comparison); only one computation of a median of $\cO(\log T)$ data. In comparison: ExtremeHunter = $\cO(T^2)$!, ExtremeETC = $\cO(\log(T)^4)$ in the best case, MaxMedian = online ranking of the data (what does this cost on average?).
	\item Efficient Storage! Can store only the $\cO(\log T)$ batch' maximum! Technically for the others all samples are needed, except ExtremeETC.
\end{itemize}

Possible drawbacks (including on the story we want to tell in the paper)

\begin{itemize}
	\item Biggest one: algorithm is not anytime!
	\item Similar idea as MaxMedian, which is also very simple. Insist on the fact that it is actually different and that we have better guarantees. 
	\item the ETC idea can seem a poor solution to some people, as if we're wrong we suffer full regret.
\end{itemize}

\subsection{MoMax}

\subsubsection{Properties of the maximum of $n$ random variables}

Consider a collection of i.i.d random variables $(X_1, \dots, X_n)$ 
with cdf $F_X$ and denote $G_X=1-F_X$ and 
$X_n^+ = \max \{X_1, \dots, X_n \}$. Then the cdf of $X_n^+$ 
is immediately derived from F, for any $x \in \R$,

\begin{equation}\label{eq::prob_inf}\bP(X_n^+ \leq x)= F_X(x)^n \leq \exp(-n G_X(x)) \;.
\end{equation}

We see that $\bP(X_n^+ \geq x)$ have a more complicated form. 
However, when $x$ is large a simple union bound is actually quite tight,
\begin{equation}
\label{eq::prob_sup}
\bP(X_n^+ \geq x)\leq \sum_{i=1}^n 
\bP(X_i\geq x) = n G(x) \;.
\end{equation}
Using Equation~\ref{eq::prob_inf} and \ref{eq::prob_sup}, for two samples $(X_1, \dots, X_n)$ and $(Y_1, \dots, Y_n)$ with respective maxima $X_n^+$ and $Y_n^+$ we want to upper bound the probability $\bP(X_n^+ \leq Y_n^+)$ by finding a suitable sequence $x_n$ aimed at minimizing $\max(\bP(X_n^+ \leq x_n), \bP(Y_n^+ \geq x_n))$. We start by providing a result for some parametric assumptions on the tail of the distributions, showing that in this case an upper bound in $\cO((\log n)^{l+1} n^{-l})$ can be obtained for some $l>0$.

\begin{definition}
Arm $k$ is exponential if $G_k(x) \sim a_k e^{-\lambda_k x}$
\end{definition}

{\color{blue} better statement of this result for making it clear that $X$ is the distribution with the heavier tail}

\begin{lemma}[Concentration for exponential and polynomial tails]
\label{lem::concent_expoly_app} 
Consider two tails that are either polynomial or exponential 
with parameters $\lambda_1 < \lambda_2$. Let $X_n^+$ 
and $Y_n^+$ denote respectively the maximum of $n$ i.i.d 
random variables drawn respectively from $\nu_X$ 
(with parameeter $\lambda_1$) and $\nu_Y$ 
(with parameter ($\lambda_2$). Then, 
there exists some sequence $x_n$ for which 
	\[
	\max\left\{\bP\left(X_n^+ \leq x_n\right), 
	\bP\left(Y_n^+\geq x_n \right) \right\} 
	= \cO\left(\frac{(\log n)^{\lambda_2/\lambda_1}}{
	n^{\frac{\lambda_2}{\lambda_1}-1}}\right) \;.
	\]
\end{lemma}

\begin{proof}
The key of the proof is to consider $x_n$ "slightly" 
below $G_X^{-1}(1/n)$. Consider the exponential tails first: we say 
that the tails are exponential if there exist parameters 
$(a_1, a_2, \lambda_1, \lambda_2)$ such 
as for $x$ large enough, $G_X(x)=a_1 \exp(-\lambda_1 x)$ 
and $G_Y(x)=a_2 \exp(-\lambda_2 x)$, 
with $\lambda_1 < \lambda_2$. The closest 
equivalent of the gap in classical bandits is 
the quantity $l_{12}= \frac{\lambda_2}{\lambda_1}-1$. Then, we 
choose 
\[
x_n = \frac{1}{\lambda_1}\left(\log n + \log(a_1) 
- \log(l_{12} \log n)\right) \;.
\]
	
	We now simply compute $G_X(x_n)$ and $G_Y(x_n)$. First,	
	\begin{align*}
	G_X(x_n) &= a_1 \exp(-(\log n + \log a_1 - \log(l_{12})\log n))\\
	& = \frac{l_{12}(\log n)}{n} \;.
	\end{align*}
	Then, 
	\begin{align*}
	G_Y(x_n) &= 
	a_2 \exp\left(-\frac{\lambda_2}{\lambda_1}
	\left(\log n + \log a_1 - \log(l_{12}\log n\right)\right) 
	\\
	& = \frac{1}{n^{\frac{\lambda_2}{\lambda_1}}} 
	\times (l_{12} \log n)^{\frac{\lambda_2}{\lambda_1}}
	\times\frac{a_2}{a_1^\frac{\lambda_2}{\lambda_1}}
	\end{align*}

	So finally, using Equation~\ref{eq::prob_inf} and \ref{eq::prob_sup} we obtain 
	\[
	\bP\left(Y_n^+ \geq x_n\right) 
	= \cO\left(\frac{(\log n )^{\frac{\lambda_2}{\lambda_1}}}
	{n^{l_{12}}}\right) \quad \text{and} \quad 
	\bP\left(X_n^+ \leq x_n\right) \leq \frac{1}{n^{l_{12}}} \;, 
	\]
which gives the result.
	

Now we consider polynomial tails, that we parametrize this time as $G_X(x)=a_1 x^{-\lambda_1}$ and $G_Y(x)=a_2 x^{-\lambda_2}$. We follow the exact same proof, this time with the sequence 
\[
x_n = (a_1 n )^\frac{1}{\lambda_1} 
\times (l_{12} \log n)^{-\frac{1}{\lambda_1}} \;,
\]
with the same definition of $l_{12}$. We again have $\exp(-nG_X(x_n))=n^{-l_{12}}$, and $nG_2(x_n) = \cO\left(\frac{(\log n )^{\frac{\lambda_2}{\lambda_1}}}{n^{l_{12}}}\right)$, giving the result.

\end{proof}

\begin{remark}
	An open question could be to determine if there exists a better rate, possibly by directly computing $\bP(X_n^+ \leq Y_n^+)$ instead of using this decomposition. Indeed, with this technique it appears clearly that the order cannot be improved as the upper bounds would evolve in an opposite direction when changing $x_n$. Could be interesting to verify this with plots.
\end{remark}

Lemma~\ref{lem::concent_expoly} will be crucial to design and evaluate the performance of the MoMax-ETC strategy. It is sufficient to handle all the cases for which algorithms exist in the literature. More precisely, existing solutions work only when the growth rates of the maxima can be clearly distinguished, e.g when tails are exponential or Pareto with different rates $\lambda_X \neq \lambda_Y$. In the following, we try to relax this condition and study a looser property for tail comparison.

%{\cxolor{blue} est-ce qu'on aurait pas envie de dire asymptoticallt dominating arm-tail pour qu'on comprenne un peu mieux que c'est au niveau des queues qu'on s'intéresse aux distributions.}
\begin{definition}[Asymptotically dominating arm]
Let $F_X$ and $F_Y$ be the cumulative distribution 
functions of two distributions $\nu_X$ and $\nu_Y$. 
	We say that $\nu_X$ dominates $\nu_Y$ asymptotically 
	if there exists some constant $C>1$ and some 
	$x \in \R$ satisfying $\forall y \geq x$, $G_X(y) > C G_Y(y)$. 
	We then denote $\nu_X \succ \nu_Y$.
\end{definition}

\begin{lemma}[Concentration under Asymptotic dominance]\label{lem::prob_dominance_app}
	Consider two distributions $\nu_X$ and $\nu_Y$ satisfying $\nu_X \succ \nu_Y$. Let $X_n^+$ and $Y_n^+$ denote respectively the maximum of $n$ i.i.d random variables drawn respectively from $\nu_X$ and $\nu_Y$. Then, there exists some $\epsilon>0$ and some sequence $u_n$ satisfying $\bP(X_n^+\leq u_n) \leq 1/2-\epsilon$ and $\bP(Y_n^+\geq u_n) \leq 1/2-\epsilon$ for $n$ large enough.
\end{lemma}

\begin{proof}
We start by considering $v_n = F_X^{-1}((1/2)^{1/n})$. By construction, this sequence then satisfies $\bP(X_n^+\leq v_n)=1/2$, and for $n$ large enough the condition holds in $v_n$. We now consider

\begin{align*}
\bP(Y_n^+ \leq v_n) & = F_Y(v_n)^n \\
& =(1-G_Y(v_n))^n \\
& \color{blue}{\geq (1- \frac{1}{C} G_X(v_n))^n} \\
& = \left(1-\frac{1}{C} \left(1-\left(\frac{1}{2}\right)^{1/n}\right)\right)^n \;. 
\\
\end{align*}
{\color{blue}question par rapport à la ligne en bleue: ici tu as utilisé que $v_n$ tend vers +  infiny donc existee n large enough pour etre dans lee régime de domination asymptotique c'est ça ?}


Now we can consider the asymptotic behavior of this quantity, using first that $1- \frac{1}{2^{1/n}} \sim \frac{\log 2}{n}$, and deducing then that \[\left(1-
\frac{1}{C} \left(1-\left(\frac{1}{2}\right)^{1/n}\right)\right)^n \sim \frac{1}{2^{\frac{1}{C}}}>\frac{1}{2} \;.\]

So for $n$ large enough we have both $\bP(X_n^+ \leq v_n)=1/2$ and $\bP(Y_n^+\leq v_n)\geq 1/2+\epsilon'$ for some $\epsilon'$ that depends on $C$. As there is a strictly positive gap between these two quantities, we can find some $\epsilon>0$ and a sequence $u_n$ satisfying both $\bP(X_n^+ \leq u_n)=1/2-\epsilon$ and $\bP(Y_n^+\leq u_n) \geq 1/2 + \epsilon$. The maximum possible value for $\epsilon$ depends only of the parameter $C$. This concludes the proof.
\end{proof} 

\begin{remark} We could ask ourselves if it is possible to obtain the same result with an even stronger condition, for instance only assuming $G_1(x)>G_2(x)$ for $x$ large enough. However, with this assumption it is possible to build pathological cases, such as defining $G_1(x)=G_2(x)\left(1+\frac{1}{x}\right)$. With the same analysis as the proof of Lemma~\ref{lem::prob_dominance}, by replacing $C= 1+\frac{1}{v_n}$ we would obtain $2^{-\frac{v_n}{v_n+1}} \rightarrow_{n \rightarrow + \infty} 1/2$. Logically, the two tails because impossible to distinguish when $n\rightarrow + \infty$. 
\end{remark}

\subsubsection{Concentration of the MoMax} 

\begin{lemma}[Concentration of MoMax]
\label{lem::MoMax_concentration_appendix}
Consider a sample of $m \in \N$ batches containing 
$n\in \N$ observations each. The $n\times m$ 
observations $(X_1^1, \dots, X_n^m)$ are i.i.d and 
drawn from a distribution $\nu_X$. For all $i \in [1, m]$ 
we denote $X_{n}^{i, +}$ as the maximum 
over the $n$ observations of the $i$-th batch, 
and $\bar X_n^+$ as the median of $(X_{n}^{i, +})_{i \leq m}$, that 
we call "Median of Maxima" (MoMax) of the 
sample. Then, for any $(x, y) \in \R^2$ satisfying 
respectively $\bP(X_n^{1, +} \geq x) < 1/2$ 
and $\bP(X_n^{1, +} \leq y) < 1/2$, it holds that 
	\[
	\bP(\bar X_n^+ \geq x) \leq 
	\exp(-m \times\kl(1/2, \bP(X_n^{1, +}\geq x))) \;,
	\]
	and  
	\[
	\bP(\bar X_n^+ \leq y) \leq 
	\exp(-m \times \kl(1/2, \bP(X_n^{1, +}\leq y))) \;,
	\]
where for $(p, q) \in (0, 1]$, $\kl(p, q)= p\log(p/q)+(1-p) \log((1-p)/(1-q))$, is the KL-divergence between two Bernoulli distributions with parameters $p$ and $q$.
\end{lemma}

\begin{proof}
Using the same kind of demonstration as \cite{bubeck_heavy} for the \textit{Median of Means} estimator, we use the concentration of Bernoulli random variables. The intuition is the following: if the median of the samples is larger (resp. smaller) than some $x \in \R$, then it holds that at least half of the batch estimators are larger than $x$ (resp. smaller), which gives $\sum_{i=1}^m \ind(X_n^{i, +} \geq x) \geq \lceil m/2 \rceil$. Hence, we can use the classical Chernoff concentration for Bernoulli random variables

\begin{align*}
\bP(\bar X_n^+ \geq x) &\leq \bP\left(\sum_{i=1}^{m} \ind\left(X_{n}^{i, +} \geq x \right) \geq \left\lceil \frac{m}{2}\right\rceil\right) \\
& \leq \exp\left(-m \times \kl\left(1/2, \bP(X_n^{1,+} \geq x)\right)\right) \;, 
\end{align*}

which holds if $\bP(X_n^+ \geq x) < 1/2$. The second result is directly proved using the exact same argument, since $\bP(X_n^+ \leq y) < 1/2$.
\end{proof}


\begin{corollary}\label{corr::prob_momax_lose}

Consider $\bar X_n^+$ and $\bar Y_n^+$ the MoMax of two samples of sizes $m \times n$ drawn respectively from distributions $\nu_X$ and $\nu_Y$. Then,

\begin{enumerate}
	\item If $\nu_X$ and $\nu_Y$ satisfy the condition of 
	Lemma~\ref{lem::concent_expoly}, then \textbf{for any} 
	$\epsilon>0$ there exists $n_0$ %large enough satisfying for any 
	such that for any
	$n\geq n_0$, 
	\[
	\bP\left(\bar X_n^+ \leq \bar Y_n^+\right) 
	\leq 2 \exp(-m\times \kl(1/2, \epsilon)) \;.
	\] 
	\item If $\nu_X$ and $\nu_Y$ satisfy the 
	condition of Lemma~\ref{lem::prob_dominance}, then 
	\textbf{there exists} some $\epsilon>0$ and $n_0$ %large enough
	such that 
	for any $n \geq n_0$, 
	\[
	\bP\left(\bar X_n^ + \leq \bar Y_n^+\right) 
	\leq 2 \exp(-m\times \kl(1/2, 1/2-\epsilon))\;.
	\]
\end{enumerate}
\end{corollary}

\begin{proof}
Denote $X_n^+$ and $Y_n^+$ the respective maxima of a single batch of size $n$ drawn from $\nu_X$ and $\nu_Y$. 

Under the assumptions of Lemma~\ref{lem::concent_expoly}, there exists a sequence $x_n$ satisfying 
{\color{blue}typo ligne d'en dessous j'imagine que ça doit être un max et qu'il n'y a pas le terme en $\bP(X_n)$}
$\bP(X_n)\left\{\bP\left(X_n^+ \geq x_n\right), \bP\left(Y_n^+\leq x_n \right) \right\} = \cO\left(\frac{(\log n)^{\lambda_2/\lambda_1}}{n^{\frac{\lambda_2}{\lambda_1}-1}}\right) \rightarrow_{n \rightarrow + \infty} 0$. Hence, for any $\epsilon >0$ for $n$ large enough the probabilities are both smaller than $\epsilon$. We then simply notice that $\bP(\bar X_n^+ \leq \bar Y_n^+) \leq \bP(\bar X_n^+ \leq x_n) + \bP(\bar Y_n^+ \geq x_n)$, which gives the result by direct application of Lemma~\ref{lem::MoMax_concentration}.

Similarly, Lemma~\ref{lem::prob_dominance} ensures the existence of some sequence $x_n$ and some $\epsilon>0$ satisfying $\max\left\{\bP\left(X_n^+ \geq x_n\right), \bP\left(Y_n^+\leq x_n \right)\right\} \leq 1/2-\epsilon$, for $n$ large enough. 
Following the reasoning from the previous case, we obtain the result.
%The result is then direct, with the same reasoning as for the first statement.
\end{proof}

\begin{remark}

$\kl(1/2, \epsilon_n) \approx 1/2 \log(1/\epsilon_n) - \log 2$, so if we have $\epsilon_n \sim n^{-\ell}$ like the concentration for the semi-parametric tails we actually have an upper bound in $\exp(-m (\ell \log(n)-\log 2))$. This is actually more logical than in the other size: with a strong concentration or a large sample size we can reduce the batch size required!
\end{remark}	

\subsection{Upper bound on the extremal regret}

\begin{theorem}[Regret of ETC in Extreme Bandits]
\label{th::regret_ETC}
	Let $\pi$ be an Explore-Then-Commit policy requiring 
	$N_0(T)$ samples for each arm before 
	committing to a single arm. Consider any bandit 
	problem $\nu=(\nu_1, \dots, \nu_K)$ with an asymptotically 
	dominating arm $\nu_1$, and denote $(X_1, \dots, X_n, \dots)$ 
	the observations sequentially collected from 
	this arm during the game. When $T$ is large enough 
	the extreme regret of ETC satisfies
	\begin{align*}
	\cR_{T}^\pi &= \bE\left[\max_{n \leq T} X_n\right] - 
	\bE\left[\max_{t \leq T} X_{N_{I_t}(t)}^{I_t}\right] 
	\\
	& \leq \bE\left[\max_{n \leq T} X_n\right]  
	- \bE\left[\max_{n \leq T-KN_0(T)} X_n\right] 
	+\bP(I_T\neq 1)\bE\left[\max_{n \leq T-KN_0(T)} X_n\right] 
	\\
	& \leq \underbrace{\bE\left[\max_{n \leq T} X_n\right]  - 
	\bE\left[\max_{n \leq T-KN_0(T)} X_n
	\right]}_{\text{Exploration Cost}} 
	+ 
	\underbrace{\bP(I_T\neq 1)\bE\left[\max_{n 
	\leq T} X_n\right]}_{\text{wrong 
	arm picked error}} \;.
	\end{align*}
\end{theorem}

\begin{proof}
	The ETC simplifies a lot the study of the extremal regret, as we can separate the explore and commit phase in the analysis. First, an exact decomposition of the expected value of the policy is 
	\[
	\bE\left[\max_{t \leq T} X_{N_{I_t}(t)}^{I_t}\right] 
	= \bE\left[\max \left\{ \max_k \max_{n \leq N_0(T)} X_n^k 
	, \max_{n=[N_0(T),T-(K-1)N_0(T)]} X_n^{I_T}\right\}\right] \;.
	\]
	
	We obtain a trivial lower bound by simply ignoring the exploration phase, and further proceed by only considering the event when the arm picked for the exploitation phase is the best arm
	
	\begin{align*}
	\bE\left[\max_{t \leq T} X_{N_{i_t}(t)}^{I_t}\right] &\geq \bE\left[\max_{n=[N_0(T),T-(K-1)N_0(T)]} X_n^{I_T} \ind(I_T=1)\right] \\
	&= \bE\left[\max_{n=[N_0(T),T-(K-1)N_0(T)]} X_n \ind(I_T=1)\right] \\
	& = \bP(I_T=1) \bE\left[\max_{n=[N_0(T),T-(K-1)N_0(T)]} X_n\right] \\
	& =\bP(I_T=1) \bE\left[\max_{n=[1,T-KN_0(T)]} X_n\right] \; \\
	&=  \bE\left[\max_{n \leq T-KN_0(T)} X_n
	\right] - \bP(I_T\neq 1)  
	\bE\left[\max_{n \leq T-KN_0(T)} X_n
	\right]  \\
	& \geq \bE\left[\max_{n \leq T-KN_0(T)} X_n
	\right] - \bP(I_T\neq 1)  
	\bE\left[\max_{n \leq T} X_n
	\right] \;.
	\end{align*}
	
	{\color{blue} pour la première ligne utilisation du fait que les distributions sont à valeurs positives pour faire apparaître l'indicatrice ?
	Autre remarque, est-ce que les indices devraient aller jusuq'à $T- (K-1)
	N_0(T) -1$ plutôt ? (j'avoue que je pinaille)}
	
There second equality holds because the fact that arm $1$ is chosen by the algorithm after the exploration phase is independent of the rewards that are available for arm $1$ in the exploitation phase. This concludes the proof.
\end{proof}



\paragraph{Examples: Polynomial and Logarithmic tails} 
From \cite{bhatt2021extreme} Equation (10), for a polynomial tail with 
rate $\alpha$ we obtain 
\[
\frac{\bE[\max_{n \leq T-KN_0(T)} X_n]}{\bE[\max_{n \leq T} X_n]} 
\sim \left(1-\frac{KN_0(T)}{T}\right)^\frac{1}{\alpha} \;, 
\]
or 

\[
\bE \left[\max_{n \leq T-KN_0(T)} X_n\right]-\bE[\max_{n \leq T} X_n] 
= (cT)^{1/\alpha}\times \left[1-\left(1-\frac{KN_0(T)}{T}\right)^{1/\alpha}\right]\sim \frac{C^{1/\alpha} K N_0(T)}{\alpha T^{1-1/\alpha}} 
\]

For a logarithmic tail $a e^{-\lambda x} $, 
we have 
{\color{red} ça vient d'où ça ?}
\[
\frac{\bE[\max_{n \leq T-KN_0(T)} X_n]}{\bE
[\max_{n \leq T} X_n]} \sim 
\frac{\log(T-KN_0(T))+\log a}{\log T + \log a} = 1 
+ \frac{\log\left(1-K\frac{N_0(T)}{T}\right)}{\log T 
+ \log a} \;, 
\]
or 
\[
\bE\left[\max_{n \leq T-KN_0(T)} X_n\right]
-\bE[\max_{n \leq T} X_n] = 
-\frac{\log\left(1-\frac{KN_0(T)}{T}\right)}{\lambda} 
\sim \frac{K N_0(T)}{\lambda T} \;.
\]

Hence, we see that the exploration cost vanishes in both cases if $N_0(T) = o(T^\delta)$ for any $\delta>0$. The exponential tails are less restrictive as $N_0(T)=o(T)$ is enough.

{\color{red} est-ce qu'on veut rajouter le statement de l'espeerance du max avec des distrib exponentielles pour justifier le statement de la ligne au dessus}

%{\color{blue} TODO Yo: j'ai pas encore checké cette partie là (au dessus).}

We now consider specifically the probability 
$\bP(I_T\neq 1)$ of MoMax-ETC. For 
simplicity we denote by $\bar X^{k, +}$
the MoMax estimator of arm  $k$ at the end of 
the exploration phase. Here, we assume either the 
tail assumptions of Lemma~\ref{lem::concent_expoly} 
or Lemma~\ref{lem::prob_dominance} and denote simply 
as $(m_T, n_T)$ the batch size and sample size used 
in MoMax. We have
\begin{align*}
\bP(I_T \neq 1) =& \sum_{k=2}^K \bP(I_T=k) \\
\leq & \sum_{k=2}^K \bP(\bar X^{1, +} \leq \bar X^{k, +}) \;.
\end{align*}

We then deduce from Corollary~\ref{corr::prob_momax_lose} 
that under assumptions of Lemma~\ref{lem::concent_expoly}, for 
any $\epsilon>0$ if $n_T$ is large enough we obtain 
\[
\bP(I_T \neq 1) \leq 2K \exp(-m_T\kl(1/2, \epsilon)) \;.
\]

Similarly, under the assumptions of 
Lemma~\ref{lem::prob_dominance} there exists 
some $\epsilon>0$ such that if $n_T$ is large enough we obtain 
\[
\bP(I_T \neq 1) \leq 2K \exp\left(-m_T\kl(1/2, 1/2-\epsilon)\right) \;.
\]

{\color{blue} pourquoi c'est $n_T$ que tu tunes ici ? c'est $m_T$ le nombre de batch sur lequel on a envie de jouer ici non?}

In the first case it suffices to choose $n_T = \frac{\log T}{\kl(1/2, \epsilon)}$ to obtain a probability of order $T^{-1}$, and $\epsilon$ can be chosen by the learner. In the second case $\epsilon$ is not known by the learner and so we have to choose $m_T$ satisfying $\log T = o(m_T)$ to obtain an upper bound of $T^{-1}$ asymptotically.


\begin{remark}[Regret of ExtremeHunter]
The regret of ExtremeHunter is of order $\bE[R_T] = \bE[\max_T X_n] \times \cO\left(T^{-\frac{b}{(b+1)\alpha^\star}}\right)$. This quantity is not vanishing when $T\rightarrow +\infty$ because it provides a scaling in $T^\frac{1}{(b+1)\alpha^*}$. On the other hand, the interest of the analysis of ExtremeHunter is that it provide an upper bound on the expected number of pulls of sub-optimal arms, of order $\cO\left(\right)$. 

Note that there is an inconsistency between different notations in the paper and in the code. Is $\log^2(n) = \log \log n $ ? It seems that Mastane thinks so. If so why do they write $\exp(-\log^2(n))$ in $\delta$ and not $1/\log(n)$? The value of $N$ is like $\cO(\log n)^{4+2/b}$, because of two conditions: one with a $\log^2(n)$ and the other with a $\log(n)^2$. If we take $\log^2(n)$ as $(\log(n))^2$ we indeed need $4+2/b$, if it is $\log\log$ then we need $(\log \log n)^4$ and $\log(n)^{2+1/b}$... which is the value of $N$ Michal put in the code... 
{\color{green}also check guaranties données dans le papier de Mastane pour le regret de ExtremeHunter histoire de voir si ils ont un résultat plus fort, il me semble que oui}

\end{remark}

==> concentration_section.tex <==
%\section{COMPARING (QUANTILE) of MAXIMA}
\section{COMPARISON OF MAXIMA}
\label{sec::max_comp}
%In this section we provide different results on the outcome of the comparison between the respective maxima of two samples drawn from different arms. We first introduce two kind of assumptions that we will make on their distributions, and then investigate what can be said of such comparison under those assumptions. We will then motivate and introduce Quantile of Maxima (QoMax), and detail the properties of this estimator.

In this section, we provide some results for the pairwise-comparison of the maximum of $n$ samples coming from two different arms. This motivates the introduction of Quantile of Maxima (QoMax) the estimator used in the algorithms we propose.

%\subsection{Preliminary definitions}

%Following the line of work of \cite{bhatt2021extreme}, we aim at providing an algorithm that requires little knowledge on the arm's distribution to be implemented. %However we also want to investigate the theoretical property of our algorithms, and to do so it is necessary to establish which kind of problems we want to analyze.
As the focus of this work is related to the tails of the reward distributions, it is natural to consider
%As we will look at the upper tails of the distributions, we define
the \textit{survival function} (\ccdf in the rest of the paper) $G$ of a distribution $\nu$, that we define as
\[
\forall x \in \R, \quad
G(x)=\bP_{X\sim \nu}(X \geq x) \;.
\]
We introduce two different assumptions that we will consider for the distribution of the arms. %Those assumption are inspired by existing works focusing on semi-parametric distributions.
%Throughout the paper, we will consider two different assumptions for the distribution of the arms. Inspired by the existing literature focusing on semi-parametric distributions, we define the following.

\begin{definition}[Exponential or polynomial tails]\label{def::tails}
Let $\nu$ be a distribution of \ccdf $G$. If there exists $C>0$ and $\alpha > 1$ such that $G(x) \sim_{x \rightarrow \infty} 
Cx^{-\alpha}$ we say that $\nu$ has a \textbf{polynomial tail}.
% rajout when x tends to \inf

If there exists $C\in \R, \lambda \in \R^+$ such that $G(x)  \sim_{x \rightarrow \infty}
C \exp(-\lambda x)$ we say that $\nu$ has an \textbf{exponential tail}.
\end{definition}

We call these assumptions \textit{semi-parametric} as nothing is assumed on the lower part of the tail, %before some unknown quantile,
%hence the term of \textit{semi-parametric distribution}.
We remark that assuming a polynomial tail is a weaker condition than the second-order Pareto assumption from \cite{carpentierExtreme}. Now, we consider a much more general assumption characterizing the comparison between the tails of two distributions.
%
\begin{definition}[Dominating tail]
\label{def:asympt_dominating}
Let $G_1$ and $G_2$ be the \ccdf of two distributions $\nu_1$ and $\nu_2$.
We say that the tail of $\nu_1$ \textbf{dominates} the tail of $\nu_2$ (denoted $G_1 \succ G_2$)
if there exists some $C>1$ and
$x \in \R$ satisfying
$\forall y \geq x$,
\[
G_1(y) > C G_2(y)\;.
\]
\end{definition}
%

In a $K$-armed bandit, assuming that one arm's tail dominates the others avoid the pathological cases introduced in \cite{nishihara2016no}, where no strategy can achieves a vanishing regret. In particular, it ensures that for $T$ large enough one arm can be identified as the \textit{best arm} for the Extreme Bandit problem. To the best of our knowledge, it is the weakest assumption introduced so far in this setting.

\subsection{Properties of the Maximum of Random Samples}\label{sec::prop_max}
We now establish some properties for comparing
the maxima of random samples of the same size
drawn from different distributions. All proofs are reported in Appendix~\ref{app::prop_maximax}.
We first consider $n$ i.i.d random
variables $(X_1, \dots, X_n)$ drawn from a distribution $\nu$
of \ccdf $G$, and define
$X_n^+ = \max \{X_1, \dots, X_n \}$.
The cdf of $X_n^+$
is directly derived from $G$ and for all $x\in \R$ as
\begin{equation}
\label{eq:prob_inf_main}
\bP(X_n^+ \leq x)= (1-G(x))^n \leq \exp(-n G(x))\;.
\end{equation}
We can also upper bound the \ccdf of $X_n^+$ as
\begin{equation}
\label{eq:prob_sup_main}
\bP(X_n^+ \geq x)\leq \sum_{i=1}^n
\bP(X_i\geq x) = n G(x) \;.
\end{equation}
These two simple inequalities will be useful to prove the next results, and are sufficient because they are quite tight for large values of $x$.

Now consider another sample $(Y_1, \dots, Y_n)$ drawn from a distribution of \ccdf $G'$, and $Y_n^+= \max \{Y_1, \dots, Y_n \}$. Using Equation~\eqref{eq:prob_inf_main} and \eqref{eq:prob_sup_main} we want to
upper bound the probability $\bP(X_n^+ \leq Y_n^+)$
by finding a suitable sequence $x_n$ aimed
 at making $\bP(X_n^+ \leq x_n)$ and $\bP(Y_n^+ \geq x_n))$ as small as possible. We consider first the semi-parametric case.

\begin{lemma}[Comparison of Maxima]\label{lem::max_comp}
Let $G$ and $G'$ be the \ccdf of two distributions $\nu$ and $\nu'$, satisfying $G \succ G'$. Denote by $X_n^+$ and $Y_n^+$ the maxima of two random samples of size $n$ drawn from $\nu$ and $\nu'$. Then, for any $q\in (0, 1)$ there exists $n_{G, G'}\in \N$, a sequence $x_n$, and some $\epsilon>0$ satisfying $\forall n \geq n_{G, G'}$,
\[\bP(X_n^+\leq x_n) \leq q-\epsilon \;,\text{ and} \quad \bP(Y_n^+ \leq x_n)\geq q+\epsilon\;.\]
If we further assume that the two tails are either polynomial or exponential, with resp. second parameter $\lambda$ and $\lambda'$, and define $\delta = \frac{\lambda}{\lambda'}-1$. If $\delta>0$, $x_n$ and $n_{G, G'}$ can be chosen to satisfy
\[
\max\{\bP(X_n^+\leq x_n), \bP(Y_n+ \geq x_n)\}
= \cO \left(\frac{(\log n)^{\delta+1}}{n^\delta}\right)\;.
\]
\end{lemma}

Lemma~\ref{lem::max_comp} is a crucial result in our study. Indeed it shows that even under the stronger semi-parametric assumption, $\bP(X_n^+\leq Y_n^+)$ do not decrease as fast as what we usually obtain from concentration theory in the classical bandit setting. Furthermore, the rate $\delta$ is problem-dependent and can be arbitrarily small. As pointed out by \cite{carpentierExtreme} it can actually be seen as the Extreme Bandits equivalent of the \textit{gap} in bandits, we therefore call $\delta$ the \textbf{\textit{tail gap}}. Furthermore, we prove in Lemma~\ref{lem::prob_lower} (in Appendix) a lower bound of order $\cO(n^{-(1+\delta)})$, which definitely motivates using more robust statistics on the distributions' tails.

\subsection{Quantile of Maxima (QoMax)}

Results similar as those of Section~\ref{sec::prop_max} have been previously encountered in bandit literature. In \citep{bubeck_heavy}, the authors study the problem of bandit with heavy tails: they first prove a concentration inequality in $n^{-\epsilon}$ for some $\epsilon>0$  and use this result to build several estimators with faster convergence. Among them, they consider %a truncation-based estimator and
the Median-of-Means (MoM) introduced by \cite{alon1999space}. %Without strong assumption, truncation does not seem well suited for Extreme Bandits.
We build a natural variant of MoM, that we call Quantile of Maxima (QoMax). The principle of QoMax is simple: the learner chooses a quantile $q$, and has access to $N = b \times n$ data. It then allocates the data in $b$ batches of size $n$ and: (1) find the maximum of each batch, (2) compute the quantile $q$ over the $b$ maxima. We summarize QoMax in Algorithm~\ref{alg::qomax}.

\begin{algorithm}[hbtp]
	\SetKwInput{KwData}{Input}
	\KwData{quantile $q$, $b$ batches of size $n$, $(X_1^i, \dots, X_n^i)_{i \leq b}$}
	\For{$i=1, \dotsc, b$}{Compute $(X_n^+)^i=\max \{X_1^i, \dots, X_n^i \}$}
	\SetKwInput{KwResult}{Return}
	\KwResult{quantile of order $q$ of $\{(X_n^+)^1, \dots, (X_n^+)^b\}$}
	\caption{Quantile of Maxima (QoMax)}
	\label{alg::qomax}
\end{algorithm}

For a finite set of size $b$, we simply define the quantile $q$ as the observation of rank $\lceil bq \rceil$ in the list of sorted data (in increasing order).

\begin{remark}
In general QoMax is \textbf{not} an estimate of the expectation of the maximum. We will use it to \textbf{compare two tails}, in order to find the heaviest.
\end{remark}

Let $\kl(x, y)=x\log(x/y) + (1-x)\log((1-x)/(1-y))$ denote the KL-divergence associated with two Bernoulli distributions of parameters $x$ and $y$ in $(0, 1)$, we then establish the fundamental property of QoMax.

\begin{lemma}[Deviation inequalities for QoMax]\label{lem::QoMax_comp} Let $(X_1^i, \dots, X_n^i)_{i \leq b}$ denote $b$ batches of $n$ i.i.d samples, define $\bar X_{n, b}^q$ their $q$-QoMax, and $X_n^+=\max\{X_1^1, \dots, X_n^1\}$. For any quantile $q\in (0, 1-1/b)$ and $(x, y) \in \R^2$, %it holds that
satisfying respectively
\[\bP(X_n^+ \leq x) < q \text{, and  } \bP(X_n^+ \geq y) \leq 1-q-1/b\;,\]
then
\begin{align*}
\bP\left(\bar X_{n, b}^q \leq x \right)& \leq \exp(-b \times \kl(q, \bP(X_n^+ \leq x))), \text{and} \\
\bP\left(\bar X_{n, b}^q \geq y \right)& \leq \exp(-b \times \kl(1-q', \bP(X_n^+ \geq y)))\;,
\end{align*}
with $q'=q+1/b$.
\end{lemma}

\begin{proof} Following \cite{bubeck_heavy}, we remark that if $\bar X_{n, b}^q \leq x$ then at least $\lceil bq \rceil$ maxima over the $b$ batches are below $x$, and then use the concentration of the sum of Bernoulli random variables of probability $\bP(X_n^+\leq x)$. We then use the same arguments for the second inequality. Detailed proofs are presented in Appendix~\ref{app::prop_maximax}
\end{proof}

We can now jointly use Lemma~\ref{lem::max_comp} and ~\ref{lem::QoMax_comp} to provide results on the comparison of the QoMax of two samples from distributions with different tails.

\begin{theorem}[Comparison of QoMax]\label{th::qomax_comp} Let $\nu$ and $\nu'$ be two distributions satisfying $\nu \succ \nu'$. Define $(b, n, q)$ the batch size, sample size and quantile used to compute the QoMax $\bar X_{n, b}^q$ and $\bar Y_{n, b}^q$ respectively from i.i.d samples of $\nu$ and $\nu'$. Then, \textbf{there exists} a sequence $(x_n)_{n \in \N}$, a constant $c > 0$, and an integer $n_{\nu, \nu', q}$ satisfying for $n\geq n_{\nu, \nu', q}$,
	\[\max\left\{\bP\left(\bar X_{n, b}^q \leq x_n\right), \bP\left(\bar Y_{n, b}^q \geq x_n\right)\right\} \leq \exp(-c\times b) \;. \]
If we further assume that the tails are either polynomial or exponential with a \textbf{positive tail gap}, then the result holds for \textbf{for any} $c > 0$ and $n$ larger than some $n_{c, \nu, \nu'}$.
\end{theorem}
\begin{proof}
	The proof is detailed in Appendix~\ref{app::prop_maximax}, where we instantiate Lemma~\ref{lem::QoMax_comp} with the results obtained under the two assumptions considered in  Lemma~\ref{lem::max_comp}.
\end{proof}

The statement of Theorem~\ref{th::qomax_comp} is motivated by the analysis of the algorithms we will introduce in the next sections. However, it ensures immediately that (with the same notations) $\bP(\bar X_{n, b}^q \leq \bar Y_{n,b}^q) \leq 2\exp(-cb)$ for $n$ large enough. Strikingly, this results tells that, under the simple assumption that one tail dominates the comparison of QoMax computed with same parameters will not be in favor of the dominating arm
with a probability that \textbf{decreases exponentially with the batch size}. On the other hand $n$ just needs to be larger than some (potentially large) unknown problem-dependent constant.

\begin{remark}[Choice of quantile $q$]
The results in this section rely a lot on the minimum sample size $n_{G, G'}$ required in Lemma~\ref{lem::max_comp}, from which we can say something about the tail comparisons. Choosing $q\rightarrow 1$ (resp. $0$) will increase the relative impact of $G'$ on this sample size (resp. $G$). Without more assumptions, choosing $q=1/2$ seems appropriate. However, we will show in Section~\ref{sec::xp} that for some examples a choice of $q$ close to $1$ can be helpful.
\end{remark}

%<<<<<<< HEAD
%Guided by these results, we introduce and analyze in the next sections several Extreme Bandit strategies based on the QoMax estimator.
%=======
%Guided by these results, we now introduce and analyze several Extreme Bandit strategies based on the QoMax estimator in the next sections.
%>>>>>>> 6d525e5b4e005745c9916da6f27b457375c79cbd


==> preliminary.tex <==
\section{Outline}

For Extreme Bandits: read paper by Alexandra Carpentier, Michal for ExtremeHunter, and the "Threshold Ascent" paper. I did not perform a more recent literature review but I don't think there's much more so far. The idea is to maximize the function

\[\bE[M_n] = \bE[\max_{t \leq n} X_t^{I_t}]\;,\]

which is the maximum observed on all samples collected by the algorithm. If distributions are bounded it has been proved that not much can improve over uniform exploration (we will get closer and closer to the global upper bound anyway, input ref). We are interested in efficient solutions for unbounded distributions. We compare $\bE[G_n]$ with an oracle $G_n^\star$ with

\[\bE[G_n^\star] = \max_{k \in \K} \bE[\max_{i \in [1, T]} X_i^{k}] \;.\]

It has been proved that without further assumptions, it is possible to build arm's distributions such that the "best arm" switches with time, making the problem much harder. Hence, it is generally smart to make at least a semi-parametric assumption on the tail. In Extreme Hunter, we assume for instance the distributions to be 2nd-order Pareto. In the rest of the paper we denote $G(x) = 1- F(x) = \bP(X > x)$. The semi-parametric assumption can take the form of an exponential or polynomial tail for instance,

\begin{align*}
    G(x) &\sim a \exp(-\lambda x) \text{, or}\\
    G(x) &\sim a x^{-\alpha} \;.
\end{align*}

Note that we make this assumption \textit{for $x$ large enough}, contrarily to Extreme Hunter for instance. Hence, the distribution can take absolutely any form for smaller $x$, and we only assume an exponential/polynomial decrease in it upper tail. Still, this assumption is enough to ensure the existence of a "asymptotically dominant" arm. We want a strategy that satisfies

\[\frac{\bE[M_n]}{\bE[M_n^\star]} \rightarrow 1 \;.\]

If we want to refine this we can try to obtain a proper bound for $\bE[M_n^\star] - \bE[M_n]$. This is what they do with Extreme Hunter.

This kind of assumption seems well suited for subsampling, and we propose to adapt LB-SDA in a simple fashion.

\subsection{Some Notes on Literature}

\subsubsection{ExtremeHunter \cite{carpentierExtreme}}

Assumption = 2nd-order Pareto. Strong Parametric assumption. 4 parameters, the algorithms infers them, provide a UCB and chooses the best UCB.

\subsubsection{No Regret Bound for Extreme Bandits}

Interest of Extreme bandits for hyperparameter optimization. Cite Carpentier, and an older work (Cicirello et al, 2005). Check the latter. 

They discuss the subtleties of Extreme regret defined as the ratio of expectations, and the asymmetry when considering maximums or minimums (ex: Bernoulli distribs, where we act optimally after round 2 but the ratio does not converge to $1$).

They define the "extreme regret" as 
\[\frac{1}{T}\min_{T'\geq 1}\{T': \bE[\min_{t \leq T'} x_t^{I_t}] \leq \bE[\min_{t \leq T} x_t^\star]\} \;.\]

A distribution achieves "no extreme regret" if this quantities converges to $1$. Apparently, they are first to consider an oracle policy that is not a "single-arm" oracle.

\paragraph{Theorem 11:} For any policy, there exists a bandit problem with extreme regret larger than $K$. In my opinion this advocates for the use of semi-parametric assumptions to ensure the existence of an asymptotically dominant arm.

\subsubsection{The Max K-Armed Bandit:
A New Model of Exploration Applied to Search Heuristic Selection}

Article de Cicirello et al., 2005.

Pas très très intéressant. Proposent une heuristique Exp3, $p_i = \frac{\exp(\eta\max X^i)}{\sum \exp(\eta \max X^k)}$, suggesting $\eta \approx 1/T$. Assumptions = Gumbel distributions, pas d'analyse.

\subsubsection{A Simple Distribution-Free Approach to the
Max k-Armed Bandit Problem}

Discussion on how GEV may be viewed as the CLT of the maximum, but true distributions hardly follow GEV in reasonable horizons. Authors introduces the two assumptions (1) there is a dominant arm $i^\star$: for some $t^+$, if $t>t^+$ then one arm has a better prob to yield $t$ than all the others, (2) the gap in probability to yield $t$ increases with $t$ after $t^+$: $p_{i^\star}(t)/p_i(t) \rightarrow +\infty$.

\paragraph{ThresholdAscent} Evolving threshold $T>0$. We evaluate $S_i(T)$ the number of observations exceeding $T$ for each arm $i$.  If $\sum S_i(T) \geq s$, $T \rightarrow T+\Delta$. Then we draw the arms with the largest "Chernoff" estimator
\[i_t = \argmax U(S_i(T)/n_i, n_i) \;,\]

with $n_i$ the total number of pulls of arm $i$ and 

\[U(\mu, n) = \mu + \frac{\alpha + \sqrt{2 n \mu \alpha + \alpha^2}}{n}\;,\]

with $\alpha= \log(2nk/\delta)$. Choice of $\delta$? Ils en parlent pas...

Etude expérimentale: ils testent plein de méthodes, seule ThresholdAscent fait mieux que uniform sampling dans leurs comparaisons, d'où probablement l'abandon de ces méthodes par les auteurs suivants.


\paragraph{Extreme Bandits using robust statistics} Interesting but I think the proof is wrong. Consider the proof of Theorem 4.1 page 21. The main argument is the concentration inequality (that they call "exponential Markov inequality", but is actually Chernoff method). They essentially consider the fact that the $k/m$ order statistic ($k>m$) is larger than some well tuned value. Classically (cf MoM proofs), it is considering that a Binomial random variable with $k$ trials and a given proba has $k/m$ success. In my opinion, for the threshold they consider (which has prob $1/m^{1/\delta}$, or at least in this proof we had $-\log a_i$ to get that), we should obtain 

\[\exp(-k \kl\left(\frac{1}{m}, \frac{1}{m^{1+\delta}}\right)\;.\]

What order do we obtain? Well,

\begin{align*}
\kl\left(\frac{1}{m}, \frac{1}{m^{1+\delta}}\right) &= \frac{\delta \log m}{m} + \left(1-\frac{1}{m}\right) \log \left(\frac{1-1/m}{1-1/m^{1+\delta}} \right)\\
& \leq \delta \frac{\log m}{m} \;,
\end{align*}

for any $m$ since $m^{1+\delta}> m$. Hence, we get a concentration $\exp\left(- \frac{k}{m}\delta \log m\right)$, instead of $\exp(-k^\delta/2)$. The problem is that this expression is doubly summed on $k$ and $m$, with $k=m$ in the index. This provides at least $\sum \frac{1}{m^\delta}$, which trivially does not converge.

\subsection{Two Algorithms: MoMax-ETC and MoMax-SDA}

The first algorithm we propose is MoMax-ETC, which idea is simple:

\begin{enumerate}
	\item For each arm $k$, draw $m_T \times n_T $ rewards, allocated in $m_T$ batches of $n_T$ observations
	\item Find the maximum of each batch
	\item For an arm $k$, define its MoMax as the median of the set of its batches' maxima.
	\item Commit to the arm with the best MoMax for $T-K\times m_T \times n_T$ remaining runs.
\end{enumerate}

Characteristics of this algorithm:

\begin{enumerate}
	\item Analysis with vanishing extremal regret, tuning of $m_T$ and $n_T$ to achieve this result as a function of $T$.
	\item Computationally efficient: better than all baselines
	\item Storage efficient: store only the maxima of all batches. Can forget if $T$ is fixed, if we want to keep in case $T$ evolves (doubling trick), we store the maxima of all batches: $m_T \times K$.
\end{enumerate}

The MoMax-ETC is computationally appealing and has strong asymptotic guarantees. However, in practice the performance can vary a lot according to the constant terms below the order of magnitude of $m_T$ and $n_T$. We would prefer to build an algorithm that would be more robust, and preferably be anytime. For this reason we simply adapt the LB-SDA algorithm with MoMax comparisons instead of means comparisons. This leads to the  MoMax-SDA algorithm. Assume that for each arm $k$, $m_k(T)$ batches of $n_k(T)$ observations are available, the MoMax-SDA follows the steps

\begin{enumerate}
    \item Compute the leader $\ell(r) = \argmax n_k(r)$, as in LB-SDA (arm with max pulls). Change: tie broken in favor of best max. We take $n_k(r)$ instead of $N_k(r)=n_k(r) \times m_k(r)$.
    \item Organize $K-1$ duels: Check forced exploration, indexed on $n_k(r)$. (1) the challenger competes with the MoMax of its full history. (2) The leader use subsampling on the two levels, and computes a MoMax keeping $m_k(T)$ batches of $n_k(T)$ observations.
    \item Each wining challenger xor the leader is pulled
\end{enumerate}

Notes: 
\begin{itemize}
	\item We see that it is sufficient to make the batch size of the leader grow just as the batch size of the second most pulled arm. I think that this is a good idea to keep it like that to reduce the storage cost, see how I implemented that. 
	\item Storage can be made quite efficient, as we can only keep "rolling maxima" (again, see implementration). If we have $m$ batches of $n$ observations, I think we get like $m \times \log(n)$ observations to store on average: much more efficient than the other benchmarks (store all rewards).
	\item Computation time is not very large thanks to this efficient storage that allow to optimize querying subsample maxima.
	\item From preliminary experiments the practical performance is quite good. 
\end{itemize}


A few remarks, compared with traditional SDA:
\begin{itemize}
    \item No notion of "asymptotic optimality" in this setting, no lower bound either. Furthermore, this can be a contribution if we want to do that.
    \item From the previous point, there is no clear limit to forced exploration. To the best of my understanding we could as well ask for $\cO(T^\beta)$ for some $\beta <1$. But it is not clear what is actually \textit{needed}. FE that tends to $\infty$ seems just inevitable to ultimately reach the upper tail, and not getting stuck in the part of the distribution we don't
\end{itemize}

==> proof_draft.tex <==
\newpage

\section{MoMax-SDA}\label{app::proof_sda_brouillon}


In this section we present Momax-SDA, a combination of the LB-SDA algorithm and the MoMax trick for maxima comparison.
 
\subsection{Regret decomposition with a low probability event}

We present a first general decomposition of the 
extremal regret, that applies to any policy 
and any family of distributions.

\begin{lemma}[Regret decomposition with a low probability event]\label{lem::regret_decompo_SDA}
Consider a bandit problem $\nu=(\nu_1, \dots, \nu_K)$, assume 
that for $T$ large enough $\nu_1$ is the dominant 
arm and denote by $X_1, \dots, X_T$ i.i.d random 
variables following $\nu_1$.
We define the event $\xi_T$, dependent 
of the trajectory of the bandit algorithm as  
$$\xi_T := \{N_1(T) \leq T-KM_T\}$$ 
for some sequence $(M_T)_{T \in \N}$. Then, for 
any bandit strategy $\pi$, any constant $x_T\in \R$ it holds that

\[\bE[R_T^\pi] \leq \underbrace{\bE[\max_{n \leq T} X_n] - 
\bE[\max_{n \leq T- K M_T} X_n]}_{\text{Exploration Cost}} 
+ \underbrace{x_T \bP_{\pi}(\xi_T) 
+ \bE\left[\max_{n\leq T} X_n 
\ind(\max_{n\leq T} X_n \geq x_T)\right]}_{\text{Cost 
incurred by } \xi_T} \;.\]
\end{lemma}

\begin{proof}
\begin{align*}
\bE \left[\max_{n \leq T} X_n^{I_n} \right] 
& \geq \bE\left[\max_{n \leq N_1(T)} X_n \right] 
\quad (\textnormal{keeping observations from a single arm})
\\
& \geq  \bE \left[\max_{n \leq N_1(T)} X_n \ind(\xi_T^c)\right] \\
& \geq  \bE \left[\max_{n \leq T-KM_T} X_n \ind(\xi_T^c)\right]
 \\
& = \bE \left[\max_{n \leq T-KM_T} X_n\right] - 
\bE \left[\max_{n \leq T-KM_T} X_n \ind(\xi_T)\right] \\
& \geq \bE\left[\max_{n \leq T-KM_T} X_n\right] - 
\bE \left[\max_{n \leq T} X_n \ind(\xi_T)\right] \;.
\end{align*}

At this step the decomposition is very 
similar to the one of the ETC proof. However, this time 
the event $\xi_T$ is not independent on the 
maximum on the available rewards so we need 
to control the expectation more precisely. We use 
the notation $X_T^+ = \max_{n\leq T} X_n$ for simplicity, and
then consider a constant $x_T \in \R$ and write

\begin{align*}
\bE\left[\max_{n \leq T} X_n \ind(\xi_T)\right] 
& = 
\bE[X_T^+ \ind(\xi_T)]
\leq  \bE[X_T^+ \ind(\xi_T) \ind(X_T^+ \leq x_T)] 
+ \bE[X_T^+ \ind(\xi_T) \ind(X_T^+ \geq x_T)] 
\\
& \leq x_T \bP(\xi_T) + \bE[X_T^+ \ind(X_T^+ \geq x_T)] \;.
\end{align*}
This concludes the proof.
\end{proof}

Before going further with this result, we can make a few remarks.

\begin{remark}[Comparison with the regret bound for ETC strategies]
	The expression we obtain can be compared with the result for the ETC strategies. The first part (exploration cost) is similar, with $M_T$ as the total number of samples collected during the exploration phase. The second term is more complicated as we simply had $\bP_\pi(\xi_T) \bE[\max_{n\leq T} X_T]$ for the ETC strategy. We now require this decomposition because the event $\xi_T$ is now potentially correlated with all rewards from arm $1$, and unfortunately the last term (which is not very tight as obtained by "forgetting" $\xi_T$ on this side) will make us lose a scaling in the final bound. 
	
	However, if we look back at the term 
	\[
	\bE\left[\max_{n \leq T} X_n \ind(\xi_T)\right] = 
	\bP(\xi_T) \bE\left[\max_{n \leq T} X_n |\xi_T\right]\;,
	\]
	we see that if we were able to prove that $\bE[\max_{n \leq T} X_n|\xi_T]\leq \bE[\max_{n \leq T} X_n]$ then we would obtain the same bound as the ETC strategy. Should this result be true? Intuitively yes because the event $\xi_T$ is a "bad" event for arm $1$, and should be associated with at least a relatively bad sequence of rewards (at least up to some point). Unfortunately, this seems to be rather impossible to prove as we can't say anything about the conditional distribution...
	
	Actually, we would even be glad to be able to say something like $\bE[\max_{n \leq T} X_n |\xi_T] = \cO(\bE[\max_{n \leq T} X_n])$ as we are only interested in the scaling of the regret in the Extreme Bandit problem. We could at least try to support this claim with some empirical evidences.
\end{remark}


\subsubsection{Optimizing $x_T$ in Lemma~\ref{lem::regret_decompo_SDA}}
We want to tune $x_T$ in order to make these two terms as small as possible. It appears clearly that this tuning will depend on two factors: the probability $\bP(\xi_T)$, and the scaling of the expectation (second term) in $x_T$.

\paragraph{Further work on the expectation} We first look at the second term that depends on $x_T$, which does not depend on the bandit algorithm but only on the arm's distribution. As $X_T^+ \ind(X_T^+ \geq x_T)$ is a non-negative random variable the expectation can be written as

\begin{align*}
\bE[X_T^+ \ind(X_T^+ \geq x_T)] 
&= \int_{0}^{+\infty} \bP\left(X_T^+ \ind(X_T^+ \geq x_T) > y\right) dy 
\\
& = \int_{0}^{x_T} \bP\left(X_T^+ \ind(X_T^+ \geq x_T) > y\right) dy 
+ \int_{x_T}^{+\infty} \bP\left(X_T^+ \ind(X_T^+ \geq x_T) > y\right) dy 
\\
& \leq \int_{0}^{x_T} \bP\left(\ind(X_T^+ \geq x_T) =1\right) dy 
+ \int_{x_T}^{+\infty} T \bP\left(X_1 > y\right) dy 
\\
& = x_T \bP\left(X_T^+ \geq x_T\right) 
+ T \int_{x_T}^{+\infty} \bP\left(X_1 > y\right) dy \;.
\end{align*}

\paragraph{Application to a sub-polynomial tail} Assume that for $y \in \R$ large enough, $\bP(X_1>y) \leq C y^{-\alpha}$ for some constants $C$ and $\alpha$. 

{\color{blue} there is a need to impose $\alpha> 1$ here no?}

Replacing the probabilities in the previous result we obtain 
\[
\bE[X_T^+ \ind(X_T^+ \geq x_T)] 
\leq  \frac{C}{x_T^{\alpha-1}} 
+ \frac{C}{\alpha-1} \frac{T}{x_T^{\alpha-1}} 
= \cO\left(\frac{T}{x_T^{\alpha-1}}\right)\;.
\]

Then, we can continue by assuming for instance that 
$\bP(\xi_T)= o(T^{-\beta})$ for some $\beta \in (0, 1)$. We 
now want to jointly minimize $\frac{x_T}{T^\beta}$ 
and $\frac{T}{x_T^{\alpha-1}}$. This is performed by choosing 

\[x_T = \cO\left(T^\frac{\beta+1}{\alpha}\right) \Rightarrow \bE[X_T^+ \ind(X_T^+ \geq x_T)] = \cO\left(T^\frac{1-(\alpha-1)\beta}{\alpha}\right) = o\left(T^{\frac{1}{\alpha}}\right)  \;.\]

Hence with these two assumptions, respectively 
on the probability of the event $\xi_T$ and the 
arms' tail we have $\bE[R_T] = o\left(\bE[\max_{n\leq T} X_n]\right)$, which 
is comparable with the result of \cite{carpentierExtreme}. We 
recall that their regret scale in 
$\cO\left(\bE[\max_{n\leq T} X_n] 
\times T^{- \frac{b}{(b+1) \alpha}}\right)$.

\begin{remark}[Condition for vanishing regret]
We see that the regret vanishes is $\beta(\alpha-1)>1$. If we consider that $\beta$ is fixed by the parameters of our algorithm this can be achieved for tails that are 
\begin{itemize}
	\item Polynomial with $\alpha> 1 + \frac{1}{\beta}$.
	\item Lighter than polynomial: exponential tails, gaussian tails... 
\end{itemize}	

Hence, the complexity introduced by using another policy than ETC makes us lose the property of vanishing regret only for the "heavier" Polynomial tails. On the contraty, ExtremeHunter cannot achieve vanishing regret, as the regret scales in $\cO\left(T^\frac{1}{(b+1)\alpha}\right)$
\end{remark}

\subsection{Design of $\xi_T$ and expected number of pulls}


%In Lemma~\ref{lem::regret_decompo_SDA} we ask for the event $\xi_T$ to imply an upper bound on the number of pulls of arm $1$. 

We recall $\xi_T := \{N_1(T) \leq T-KM_T\}$. 
We now provide some ideas for the analysis 
of $\bP(\xi_T)$. First, we remark that 
\[
\bP(N_1(T) \leq T- KM_T) \leq \sum_{k=2}^K \bP(N_k(T)\geq M_T)\;.
\]

It is important to define that here $N_k(T)$ tracks the \textit{number of pulls of arm $k$ \textbf{at time $T$}} (i.e after having collected exactly $T$ rewards). 

{\color{blue} in particular, we have used that $\sum_{k=1}^K N_k(T) = T$ here!}

As the algorithm works with rounds, we now introduce the notations $n_k(r)$ and $b_k(r)$ respectively for the number of \textit{queries} of arm $k$ (i.e the algorithm decide to draw arm $k$ at the end of the round, the number of times necessary to update all batches/create new batches), and for the number of \textit{batches}, both of them after the \textit{round} $r$. We remark that the number of queries is also the sample size of one batch, so we will call $n_k$ number of queries or sample size indifferently in the rest of the proof. We denote by $r_T$ the index of the round for which the number of observations equals or exceeds $T$. As at least one observation is collected at the end of the round so it holds that $r_T\leq T$. Hence, we can obtain 
\begin{align*}
\bP(N_1(T) \leq T- KM_T) &
\leq \sum_{k=2}^K \bP(n_k(r_T) b_k(n_k(r_T)) \geq M_T) \\
& \leq \sum_{k=2}^K \bP(n_k(T) b_k(n_k(T)) \geq M_T)\;,
\end{align*}

where we shifted the analysis to the round $T$. In the rest of the paper we will assume that the batch size scales sub-linearly in the number of queries: $ \forall k, b_k(n) = n^\gamma$ for some $\gamma \in (0, 1)$. We then finish this first proof with Markov inequality
\begin{align*}
\bP(N_1(T) \leq T- KM_T) 
& \leq \sum_{k=2}^K \bP(n_k(T)^{1+\gamma} \geq M_T) \\
& \leq \sum_{k=2}^K \bP(n_k(T) \geq M_T^\frac{1}{1+\gamma})\\
& \leq \sum_{k=2}^K \frac{\bE[n_k(T)]}{M_T^\frac{1}{1+\gamma}}
\end{align*}

\begin{remark}[Upper bounding $r_T$]
We can actually prove that $r_T \in \left[\left(\frac{T}{K}\right)^\frac{1}{1+\gamma}, T^\frac{1}{1+\gamma}\right]$. The lower bound corresponds to the case where all arms have been sampled equally and the upper bound if only one arm was sampled. The fact that these two extreme cases provide the range of $r_T$ is due to the convexity of the problem. \\
Is this helpful? Probably not much if we find a polylog value for $\bE[n_k(T)]$, as replacing by $\bE[n_k(T^\frac{1}{1+\gamma})]$ has the same scaling in $T$.
\end{remark}

Thanks to this trick we can now focus on upper bounding the expectation of the number of queries of each arm for $T$ rounds of MoMax-SDA, for which we will apply techniques similar to the proof of LB-SDA.

Before doing so, we can discuss the choice of $M_T$. We want to control the exploration cost $\bE[\max_{n \leq T} X_n] - \bE[\max_{n \leq T-M_T} X_n]$, while taking the $M_T$ as large as possible. 

\paragraph{Polynomial tails} Consider values $M_T = T^\lambda$, for some $\lambda \in (0, 1)$. For a polynomial tail the exploration cost would be of order $T^{\frac{1}{\alpha}+\lambda-1}$, and the cost incurred by $\xi_T$ of order $T^{\frac{1}{\alpha} - \frac{\alpha-1}{\alpha}\frac{\lambda}{1+\gamma}}$. To equalize the two we can choose 
\[
\lambda =\frac{1}{1+\frac{\alpha-1}{\alpha(1+\gamma)}} \;.
\]

The regret is then of order $T^{\frac{1}{\alpha}+\lambda-1}= T^{\frac{1}{\alpha}- \frac{\alpha-1}{\alpha(2+\gamma)-1}} = T^\frac{1}{\alpha} o(1)$.

\paragraph{Exponential tails} Assume the growth rate of the maximum is $(\log T)^\eta$ for some $\eta>0$. Then

\begin{align*}
(\log T)^\eta - \log(T-M_T)^\eta & 
= \log(T)^\eta \left(1-\left(1+\frac{\log\left(1-
\frac{M_T}{T}\right)}{\log(T)}\right)^\eta\right) \\
& \sim \frac{\eta M_T}{\log(T)^{1-\eta} T} \;,
\end{align*} 

so for any sub-linear $M_T$ this term vanishes.

\subsection{Upper bounding the number of queries for each arm}

At this step we are now able to focusing on upper bounding the expectation of $n_k(T) = \sum_{r=0}^{T-1} \ind(k \in \cA_{r+1})$, where $\cA_{r+1} \subset \{1, \dots, K\}$ is the subset of arms that are queried before the round $r+1$, after the outcomes of the duels at round $r$.

\paragraph{Notations} In the rest of the proof 
we will assume that an infinite stream of reward 
is available for each arm, in the form of a table with 
an infinite number of row and an infinite number 
of columns so that we denote these rewards by 
$(Y_{n, m}^k)_{n \in \N, m \in \N}$.
When the algorithm collects the sequence of rewards, it will draw $Y_{n, m}^k$ as the \textbf{n-th sample} of the \textbf{m-th batch} of \textbf{arm $k$}. This way, we can properly denote the sequence of rewards that we will compare when concentrating MoMax estimators. To simplify the notation,
 we define 
\begin{center}
	$\bar Y_{k, n}^+ \coloneqq$ MoMax of the table of rewards $(Y_{i, j}^k)_{i \leq n, \; j \leq b(n)}$, as the median of the maxima \textbf{over each row}, \\ where the $n$ first observations are taken per row and the $b(n)$ first columns (batches) are considered.  
\end{center}

We will not only have to consider the MoMax on the $(n, b(n))$ first observations/batches but also on subsamples. We now explain how subsampling is considered across the observations/batch dimensions: first, the subsampling on the query dimension is performed in the LB-SDA fashion: we want to use observations only between lines $n_1$ and $n_2$ in $(Y_{i,j}^k)$. Then, to subsample across batches we will simply consider the $b(n_2-n_1+1)$ first batches. To summarize, we consider the table $(Y_{i, j}^k)_{i \in [n_1, n_2], \; j \leq b(n_2-n_1+1)}$. The main interest is that we only have to specify the subset of index used for the rows of the table, hence we will symply denote the MoMax corresponding to this table of rewards as
\begin{center}
	$\bar Y_{k, n_1:n_2}^+ \coloneqq$ MoMax of the table of rewards $(Y_{i, j}^k)_{i \in [n_1, n_2], \; j \leq b(n_2-n_1+1)}$
\end{center}


\textcolor{blue}{Bon j'avoue qu'un petit tikz ça ferait plaisir, mais c'est peut-être un peu le rush pour ça.}

\paragraph{Leader} We define the leader as the arm that has been most queried: $\ell(r)=\aargmax_k n_k(r)$. The ties are broken in favor of the arm with the best MoMax, if $\max_{k} n_k(r)=n$ and two (or more) arms satisfy $n_k(r)=n$, we consider $\bar Y_{k, n}^+$ for each of them and choose the best. In case of equality the choice is random.

\paragraph{MoMax concentration} For simplicity, we will define for each arm a constant $c_k$ and assume that there exists some $n_0$ satisfying for all $n \geq n_0$ and a well chosen $x_n$, 
\begin{equation}\label{eq::concentration_SDA}\max \left\{\bP(\bar Y_{k, n}^+ \geq x_n), \bP(\bar Y_{1, n}^+ \leq x_n) \right\} \leq \exp(-c_k b(n)) \;. 
\end{equation}

\textcolor{red}{En fait c'est plus simple si on définit juste un $c$ et $x_n$ commun pour tout le monde. On peut rajouter un petit annexe pour instancier la propriété.}

{\color{blue}je suis d'accord pour les $c_k$ quiite à prendree le min de tous; mais par contre c'est certain que ça marche pour la sequence des $x_n$, en réalité il ya une séquence $x_n^k$ pour chaque bras, comment on se débrouille pour créér $x_n$ à partir des $x_n^k$}.

We proved that this is true for example for exponential or polynomial tails. We will mostly use this concentration inequality in the rest of the proof. We now develop a decomposition similar to the one proposed for LB-SDA, which is that for any function $n_0(T)$ we have
\begin{align*}
\bE[n_k(T)] &= \bE\left[\sum_{r=0}^{T-1} 
\ind(k \in \cA_{r+1}, \ell(r)= 1)\right] 
+ \bE\left[\sum_{r=1}^{T-1}\ind(k \in \cA_{r+1}, \ell(r)\neq 1)\right] 
\\ 
& \leq \bE\left[\sum_{r=0}^{T-1} \ind(k \in \cA_{r+1}, 
\ell(r)= 1, n_k(r) \leq n_0(T))\right] 
+ \bE\left[\sum_{r=0}^{T-1} \ind(k \in \cA_{r+1}, 
\ell(r)= 1, n_k(r) \geq n_0(T))\right] \\
& 
\quad 
+ \quad \bE\left[\sum_{r=1}^{T-1}\ind(\ell(r)\neq 1)\right] \\
& \leq n_0(T) + \bE\left[\sum_{r=0}^{T-1} \ind(k \in \cA_{r+1}, \ell(r)= 1, n_k(r) \geq n_0(T)\right] + \bE\left[\sum_{r=1}^{T-1}\ind(\ell(r)\neq 1)\right] \;, \\
\end{align*}
where we used that 
\begin{align*}
\sum_{r=0}^{T-1} \ind(k \in \cA_{r+1}, n_k(r) \leq n_0(T)) & \leq \sum_{r=0}^{T-1} \ind(k \in \cA_{r+1}, n_k(r) \leq n_0(T)) \\
& \leq \sum_{r=0}^{T-1} \sum_{n = 1}^{n_0(T)} \ind(k \in \cA_{r+1}, \ell(r)= 1, n_k(r)=n) \\
&  \leq \sum_{n = 1}^{n_0(T)} \left(\sum_{r=0}^{T-1}\ind(k \in \cA_{r+1}, \ell(r)= 1, n_k(r)=n)\right) \\
&  \leq \sum_{n = 1}^{n_0(T)} 1 \\
& = n_0(T) \;,
\end{align*}

as the event $\{k \in \cA_{r+1}, n_k(r) = n\}$ can only happen at one round. Now, we can upper bound the counterpart with $n_k(r) \geq n_0(T)$, using the concentration in Equation~\eqref{eq::concentration_SDA}


\begin{align*}
A &\coloneqq \bE\left[\sum_{r=0}^{T-1} 
\ind(k \in \cA_{r+1}, \ell(r)= 1, n_k(r) \geq n_0(T))\right] \\
&\leq \bE\left[\sum_{r=0}^{T-1} \ind(k \in \cA_{r+1}, \bar Y_{k, n_k(r)}^+
 \geq \bar Y_{1, n_1(r)-n_k(r)+1:n_1(r)}^+, \ell(r)= 1, n_k(r) \geq n_0(T))\right] \\
& \leq \bE\left[\sum_{r=0}^{T-1} \ind \left(\bar Y_{k, n_k(r)}^+ \geq x_{n_k(r)}, n_k(r) \geq n_0(T), k \in \cA_{r+1} \right) \right]
\\
& \quad + \quad 
\bE\left[\sum_{r=0}^{T-1} \ind 
\left(\bar Y_{1, n_1(r)-n_k(r)+1:n_1(r)}^+\leq x_{n_k(r)}, 
\ell(r)= 1, n_k(r) \geq n_0(T), k \in \cA_{r+1}  \right) \right] 
\\
& \leq \bE\left[\sum_{r=0}^{T-1}\sum_{n_k=n_0(T)}^{T-1}\ind(\bar Y_{k, n_k}^+ \geq x_{n_k}, k \in \cA_{r+1}, n_k(r)=n_k) \right]  
\\
& \quad  +\quad \bE\left[\sum_{r=0}^{T-1}\sum_{n_k=n_0(T)}^{T-1}\sum_{n=r/K}^{T-1} \ind(\bar Y_{1, n-n_k+1:n}^+\leq x_{n_k}, \ell(r)= 1, n_k(r)=n_k, k\in \cA_{r+1}, n_1(r)=n) \right] \;. \\
\end{align*}

We now use the same trick as before to reduce the double sum on $r$ and $n_k$ to only one sum, and write that


\begin{align*}
A & \leq \bE\left[\sum_{n_k=n_0(T)}^{T-1}\ind(\bar Y_{k, n_k}^+ 
\geq x_{n_k}) \sum_{r=0}^{T-1} \ind(k \in \cA_{r+1}, n_k(r)=n_k) \right] 
+ \bE\left[\sum_{n_k=n_0(T)}^{T-1}\sum_{n=r/K}^{T-1} 
\ind(\bar Y_{1, n-n_k+1:n}^+\leq x_{n_k}) \right] 
\\
& \leq \sum_{n_k=n_0(T)}^{T-1}\bP(\bar Y_{k, n_k}^+ \geq x_{n_k}) 
+ \sum_{n_k=n_0(T)}^{T-1}\sum_{n=r/K}^{T-1} 
\bP(\bar Y_{1, n-n_k+1:n}^+\leq x_{n_k}) 
\\
& \leq \sum_{n_k=n_0(T)}^{T-1}\bP(\bar Y_{k, n_k}^+ 
\geq x_{n_k}) + 
T \sum_{n_k=n_0(T)}^{T-1} \bP(\bar Y_{1, n_k}^+\leq x_{n_k}) \;.
\end{align*}

Plugging the concentration result from Equation~\eqref{eq::concentration_SDA}, one has

\begin{align*}
A \leq \sum_{n_k=n_0(T)}^{T-1}e^{-c_k b(n_k)} + T \sum_{n=n_0(T)}^{T-1} e^{-c_1 b(n)} \leq Te^{-c_k b(n_0(T))} + \frac{T^2}{2} \exp(-c_1 b(n_0(T)))  \;.
\end{align*}

Now we choose, 
$n_0(T)=\max\left(b^{-1}
\left(\frac{2 \log T}{c_1}\right), b^{-1}\left(\frac{\log T}{c_k}\right), 
n_0 \right)$. With this choice, we get
\begin{equation}
%\label{eq:A_UB}
A = \bE\left[\sum_{r=0}^{T-1} 
\ind(k \in \cA_{r+1}, \ell(r)= 1, n_k(r) \geq n_0(T))\right]  = \cO(1) \;.
\end{equation}
If we define $b(n)=n^\gamma$, using Equation~\eqref{eq:A_UB} and the decomposition for $\bE[n_k(T)]$, it holds that for some constant $C$

\begin{equation}
\bE[n_k(T)] \leq C (\log(T))^{\frac{1}{\gamma}} + \bE\left[\sum_{r=0}^{T-1} \ind(\ell(r)\neq 1) \right] + \cO(1) \;.
\end{equation}

The next step of the proof is to have a deeper look at the second term.

\subsubsection{Upper bound on $\bE\left[\sum_{r=0}^{T-1} \ind(\ell(r)\neq 1) \right]$}

We now upper bound $\bE\left[\sum_{r=0}^{T-1} \ind(\ell(r)\neq 1) \right]$. We provide a similar decomposition as in \cite{lbsda}, considering the case where arm $1$ has already been leader and the alternative. Before that we recall the following property obtained by the definition of the leader
\begin{align*}
\ell(r) = k \Rightarrow n_k(r) \geq \left\lceil \frac{r}{K}\right\rceil \;.
\end{align*}

We then define $a_r=\left\lceil \frac{r}{4}\right\rceil$, 
and write that
%
\begin{equation}
%\label{dec:Z}
\bP\left(\ell(r) \neq 1\right)= 
\bP\left(\{\ell(r) \neq 1\} \cap \cD^r\right) + 
\bP\left(\{\ell(r) \neq 1\} \cap \bar\cD^r\right)
\;,
\end{equation}
%
where we define $\cD^r$ the event under which the 
asymptotically dominating 
arm has been leader at least once in $[a_r,r]$.
$$
\cD^r = \{\exists u \in  [a_r, r] \text{ such that } \ell(u) = 1 \}.
$$
We now explain how to upper bound the term in the left hand side of Equation~\eqref{dec:Z}. 
We look at the rounds larger than some round $r_0$ that will be specified later in the proof.


We introduce a new event 
\begin{align*}
%\cD^s& =& \{\exists u \in  [a_r, s] \text{ such that } \ell_{u} = 1 \}\\
&\cB^{u} = \{\ell(u)=1, k \in \mathcal{A}_{u+1}, n_k(u)= n_1(u) \text{ for some arm } k \} \;.&
\end{align*}
%
%
%
Under the event $\cD^r$, $\{\ell(r)\neq 1 \}$ 
can only be true if the leadership 
has been taken over by a suboptimal arm at some round between $a_r$ and $r$, that is 
\begin{equation}
\{\ell(r)\neq 1\} \cap \cD^r \subset \cup_{u=a_r}^{r-1}\{\ell(u)=1, \ell(u+1)\neq 1 \} \subset \cup_{u=a_r}^{r} \cB^u \;.
\end{equation}

This is because a leadership takeover can only happen after a challenger has defeated the leader while having the same number of observations. Moreover, each leadership takeover has been caused by either (1) a MoMax of a challenger is over-performing, or (2) a MoMax of the leader is under-performing, with a sample size in each case larger than $s_r = \lceil a_r/K\rceil$. In addition, each of these MoMax can \textbf{only cost one takeover}, hence we can simply use an union bound on these events. In summary, after defining some $r_0>8$ we have that

{\color{blue} on est sur que c'est légit de faire disparaîtree la sum en $u$ quand on inclut $\mathcal{B}_u$?}
\begin{align*}
\bE\left[\sum_{r=0}^{T-1}\ind(\ell(r) \neq 1, \cD_r)\right] & \leq r_0 + \bE\left[\sum_{r=r_0}^{T-1}\left( \sum_{u=a_r}^r \ind(\cB^u) \right)\right] \\
& \leq r_0 + \bE\left[\sum_{r=r_0}^{T-1} \left(\sum_{n=s_r}^r \left( \ind(\bar Y_{1, n}^+ \leq x_n) + \sum_{k=2}^K \ind(\bar Y_{k, n}^+ \geq x_n)\right) \right)\right] \\
& \leq r_0 + \sum_{r=r_0}^{T-1} \sum_{n=s_r}^r \left(\bP(\bar Y_{1, n}^+\leq x_n) + \sum_{k=2}^K \bP(\bar Y_{k, n}^+ \geq x_n) \right) \\
& \leq r_0 + \sum_{k=1}^K \sum_{r=r_0}^{T-1} \sum_{n=s_r}^r \exp(-c_k b(n)) \\
& \leq r_0 + \sum_{k=1}^K \sum_{r=r_0}^{T-1} r \exp(-c_k b(s_r)) \\
& = \cO(1) \;,
\end{align*}

since $b(s_r) = s_r^\gamma = \Omega(r^\gamma)$. This is true if $s_{r_0} \geq n_0$, which is the condition that allows the use of the concentration inequality \ref{eq::concentration_SDA}.

We now handle the case when the asymptotically dominating arm has never been leader between $a_r$ and $r$, which implies that it has lost a lot of duels 
against the current leader at each round. We introduce
$$
\cL^r= \sum_{u=a_r}^r \ind(\cC^u)\;,
$$
with $\cC^u = \{\exists k \neq 1, \ell(u)=k, 1 \notin \cA_{u+1} \}$.
It is proved in \cite{chan2020multi} that 
\begin{equation}
\label{eq:upper_z}
\bP(\ell(r) \neq 1 \cap \bar \cD^r) \leq \bP(\cL^r\geq r/4)\;. 
\end{equation}
and the author uses the Markov inequality to provide the upper bound
\begin{equation}
\label{eq:upper_z_2}
\bP(\cL^r\geq r/4) \leq \frac{\bE(\cL^r)}{r/4}= \frac{4}{r} \sum_{u=a_r}^r \bP(\cC^u)\;.
\end{equation}
%
%
%

From this step we can refactor $\sum_{r=r_0}^r \bP(\cL^r \geq r/4)$ using the following trick from \cite{baudry2020sub},

\begin{align*}
\sum_{r= r_0}^{T-1}  \frac{4}{r} \ind(u \in [a_r, r]) & \sum_{r= r_0}^{T-1}  4 \frac{\ind(u\leq r)}{r} \ind(a_r \leq u) \\
& \leq \frac{4}{u} \sum_{r= r_0}^{T-1} \ind(a_r \leq u) \\
&  \leq \frac{4}{u} \sum_{r= r_0}^{T-1} \ind(\lceil r/4 \rceil \leq u) \\
&  \leq \frac{4}{u} \sum_{r= r_0}^{T-1} \ind(r/4 \leq u+1) \\
& \leq  \frac{4}{u}\times 4(u+1) \\
& \leq 32 \;.\\
\end{align*}

With this result we obtain that \[\sum_{r= r_0}^{T-1} \bP(\ell(r) \neq 1 \cap \bar \cD^r) \leq \sum_{r= r_0}^{T-1} \bP( \cL^r\geq r/4) \leq 32 \sum_{r=a_{r_0}}^{T-1} \bP(\cC^r) \;.
\] 

Now we can have a more precise look at $\bP(\cC^r)=\bP(\exists k \neq 1, \ell(r)=k, 1 \notin \cA_{r+1})$. We recall that we defined in the algorithm a forced exploration $f_e(r)$, ensuring that $n_k(r) \geq f_e(r)$ for any arm $k$ and any round $r$. %We then proceed with the usual trick to compare MoMax and a union bound on the possible values of the sample sizes.

\begin{align*}
\sum_{r=a_{r_0}}^{T-1} \bP(\cC^r) & 
\leq \sum_{r=a_{r_0}}^{T-1} \bP\left(\{\bar Y_{1, n_1(r)}^+ 
\leq x_{n_1(r)}\} \cup_{k=2}^K \left\{
\bar Y_{k, n_k(r)-n_1(r)+1: n_1(r)}^+ \geq x_{n_1(r)}, 
\ell(r)=k \right\}\right) 
\\
& \leq \sum_{r=a_{r_0}}^{T-1} \sum_{n = f_e(r)}^{r/2} 
\bP(\bar Y_{1, n}^+ \leq x_{n}) + \sum_{k=2}^K 
\sum_{r=a_{r_0}}^{T-1} \sum_{n = f_e(r)}^{r/2} 
\sum_{n_k=\lceil r/K \rceil}^r \bP(\bar Y_{k, n_k-n+1:n_k}^+ 
\geq x_{n}) 
\\
&  \leq \sum_{r=a_{r_0}}^{T-1} 
\sum_{n = f_e(r)}^{r/2} \exp(-c_1 b(n)) + 
\sum_{k=2}^K \sum_{r=a_{r_0}}^{T-1} \sum_{n = f_e(r)}^{r/2} 
r \exp(-c_k b(n)) \\
& \leq \sum_{r=a_{r_0}}^{T-1} \frac{r}{2} \exp(-c_1 b(f_e(r))) 
+ \sum_{k=2}^K \sum_{r=a_{r_0}}^{T-1} \frac{r^2}{2} \exp(-c_k b(f_e(r))) 
\;,
\end{align*}

{\color{blue} deuxième somme du preemier terme
s'arrête à $r/2$ parce sinon avec strictement plus que $r/2$ samples ça seerait forcément le leader c'est ça ?}

where the use of the concentration in Equation~\eqref{eq::concentration_SDA} is permitted only if $f_e(a_{r_0})\geq n_0$. Now, this result provides a sound theoretical tuning for the forced exploration parameter as a function of $b$, as choosing $f_e(r)\leq \max_k\left(\frac{4 \log r}{c_k}\right)^\frac{1}{\gamma}$ ensures 

\[\sum_{r=a_{r_0}}^{T-1} \bP(\cC^r) = \cO(1)\;. \]

Hence, we obtain the final result that for some constant $C$ it holds that

\[\bE[n_k(T)] \leq C(\log(T))^{\frac{1}{\gamma}} + \cO(1) \;,\]

under the assumptions that Equation~\eqref{eq::concentration_SDA} holds and that the forced exploration is of the same scaling as the regret, namely $f_e(r)=\Omega((\log r)^\frac{1}{\gamma})$.

\begin{remark}[Forced exploration]
	Is the forced exploration is a first-order term in the regret, we could ask the interest of not using a simple ETC strategy. The answers are that (1) obtaining an anytime algorithm is appealing in practice, furthermore it is desirable to be able to recover from mistakes (contrarily to ETC), (2) we can technically choose any constant before the polylog term without losing the asymptotic guarantees, which is a nice property too. Hence, even if the algorithm will assign $\Omega((\log T)^\frac{1}{\gamma})$ samples to each arm it will more finely choose which arm will only be pulled the amount of forced exploration and which one will be more thoroughly explored. 
\end{remark}

\begin{remark}[How Asymptotic are the results?] 
	We detailed all the terms in the $\cO(1)$, and saw that for some of them we were considering rounds after some round $r_0$, that have to satisfy the conditions (1) $r_0 \geq K (n_0+1)$ and (2) $f_e\left(\lceil r_0/K \rceil\right) \geq n_0$, defined as functions of the $n_0$ for which Equation~\ref{eq::concentration_SDA} is valid. This $n_0$ itself depend on the constants $(c_1, \dots, c_k)$ we choose, and of course of the tails of the distributions: if the tails of all arms are "close" and the dominance of the best arm happens only after a large quantile $n_0$ can be quite large. However, nothing more can be said on this constant without considering a specific problem. 
\end{remark}

\section{Comparison of computation costs and storage capacity of each algorithm}

\paragraph{Note on the storage capacity, when storing maxima for LB-SDA} Unlike the mean, we can think about smart storage tricks. For instance, for any batch/arm, all data before the global maximum can be simply forgotten. If we consider a list of observations, we can keep the list of successive global maxima when taking the list in reverse order (keep last observation, last observation larger than the previous one with its rank in the list, etc). Best scenario: last observation is the global maximum. Worst scenario: $X_1 > X_2 > \dots > X_n$, but of course very unlikely. Faire une petite étude numérique pour voir ce que ça va donner en pratique.	

\section{Other results that can be useful or not in the future}

\paragraph{Actual Exact proba} I don't know if it will be useful, but anyway 

\[\bP(\max X_{2, i} \geq \max X_{1, i}) = \bE_{X \sim F_2^n}[F_1(X)^n] = \int_{\R} n f_2(x) F_2(x)^{n-1} F_1(x)^n dx 
\]


\subsection{Prise de note réunion 6/10}

Premier a faire idée robustification c'est bhatt et compagnie. 
on s'inspire d'eux en faisant quelque chose de différent; avec une preuve juste.

Emilie: écrire à Bhatt. 

\begin{enumerate}
\item ExtremeHunter: D,E different n'a pas trop d'impact en conservant le même $B, \delta$ forced explo initiale.
-> impact de $D$ est faible $E$ Dorian. ex: exp1: nombre de pull du bras asymp. meilleur entre 8426-8437 : quasi aucun effet. 
\item Par rapport à l'expé sur les gaussiennes: (celles aveec bcp de bras Bhatt ($K=20$). Proba $1/t$ de forced explo.
Tant que tous les bras n'ont pas été tiré au moins deux fois, l'indice de chaque bras est leur minimum. ça favorise la gaussienne avec la variance la plus faible.

\end{enumerate}

Par rapport aux messages du papier;
\begin{itemize}
\item pourquoi besoin de robustifier? asymétrie de la concentration pour $\bP(\max \geq x)$ 
vs. $\bP(\max \leq x)$  -> solution MoMax.
Si rate diffeerent pour les exponentielles, on sait quantifier ces probas; cf. lemma A.1.
\item Robustification MoMax: si  on regarde un momax mainteenant; le truc cool c'est 
$\bP(\bar{X}_n^+ \geq \bar{Y}_n^+) 
\leq \exp(-b  \times \kl(1/2, \max(\bP(\bar{X}_n^+ \geq y), \bP(\bar{Y}_n^+ \leq y))
$ 
Rq: faire gaffe à mettre $b$ le nombre de batch dans la notation du momax pour la partie stat du papier. 
Deux resultats ici, dans le cas ou les disitrbutions sont exp. ou poly avecdes rates différents, on peut analyser pour n'importe quel quantile. En revanche, k'hgypothèse de domination asymptotique impose d'avoir $q=1/2$ et de regarder la médiane. Est-ce qu'on veut faire QoMax ou MoMax?
\item Pour ETC. la partie exploration dépend dee la distribution que l'on considère. Mais 
$\bP(\xi_T)$ est juste lié à la concentration du MoMax pour nous. On peut stater un resultat général pour l'uppere bound de ETC-MoMAx et dire quee du momeent que le temre exploration se gère bien on a une analyse.
\end{itemize}


{\color{red}
TO CHECK: possibilité de faire $n^2$ pour la taille de batch dans SDA, checker nombre de pull du leader dans l'analyse avec le côté aléatoire du nombre de batch ici.}



